Security Analysis and Design for TAGA: a Touch and Go Assistant in the Aerospace Domain

There is currently a drive in the aerospace domain to introduce machine to machine communication over wireless networks to improve ground processes at airports such as refuelling and air conditiong. To this end a session key has to be established between the aircraft and the respective ground unit such as a fuel truck or a pre-conditiong unit. This is to be provided by a `touch and go assistant in the aerospace domain' (TAGA), which allows an operator to pair up a ground unit and an aircraft present at a parking slot with the help of a NFC system. In this paper, we present the results of our security analysis and co-development of requirements, security concepts, and modular verification thereof. We show that by, and only by, a combination of advanced security protocols and local process measures we obtain secure and resilient designs for TAGA. In particular, the design of choice is fully resilient against long-term key compromises and parallel escalation of attacks.

==> auth-2/auth-secure-s2.tex <==

\subsection{Concept and Security}
We say a TAGA process $(P, N, M)$ is \emph{authenticated} when 
$P$ is an authenticated KE (AKE) protocol. Since AKE protocols 
allow one to securely establish a key in the presence of active 
adversaries we 
plausible that with authenticated TAGA we
can obtain some variant of secure TAGA that is sufficient for 
Secure Setup without having to rely on employing 
a authentcity of the NFC system under $M$.
that NFC system under $M$. And
also to not share the key with the GU operator.
We have to deal with the following though: without Channel Authenticity
it is not possible to obtain the synchronization/match between
the GU's and AC's NFC links and the operator's taps, and 
and hence the alignment of setting up the secure channel and the
physical connection.
and
hence, the direct match with the physical connection.

This can be solved as follows:
First, we extend protocols so that the protocol also guarantee that the 
two parties agree on their location (i.e.\ parking slot) and service. 
Second, we extend the setup process by an additional step so that
GUs (or operators) confirm to the AC that their physical setup is
complete over the channel. Since $A$ knows the
$G$ is at the same location, it can conclude the physical connection
must be with itself and not with same $A'$ of a different location.

This gives us the following notion of TAGA security:

%if we wish a
%design whose security is no longer dependent on Channel Authenticity
%do not wish to rely on channel authenticity of the channel 

\begin{definition}
Let $T$ be a TAGA process.
\item
We say $T$ guarantees \emph{Secure TAGA II} to a GU $G$ if,
whenever $G$ has a session $(S, \Gini, \Gfin, A, K)$ then 
\begin{enumerate}
\item $(K, S)$ is a secure channel between $A$ and $G$, and
\item $A$ is located at the same location (i.e.\ parking slot) as $G$.
\end{enumerate}
\item
Similarly, we say $T$ guarantees \emph{Secure TAGA II} to an AC $A$ if,
whenever $A$ has a session $(\Amid, S, G, K, c)$ then
\begin{enumerate}
\item $(K, S)$ is a secure channel between $A$ and $G$, and
\item $G$ is located at the same location (i.e.\ parking slot) as $A$.
\end{enumerate}
\item
We say $T$ guarantees \emph{Secure TAGA II} iff $T$ guarantees
Secure TAGA II to both parties, GUs and ACs.
\end{definition}


\paragraph*{Secure Setup with TAGA II.}
We say a process flow $\mcF$  
add: has confirmation of physcial setup: if ...

\begin{example}
extend .. button pressed.
\end{example}

\begin{theorem}
Let $\mcF$ be a process flow, and $T$ be a TAGA process such
that $\mcF$ includes $T$. If $\mcF$ is well-defined/satisfies
and TAGA requirements II and $T$ guarantees Secre TAGA II then 
$\mcF$ guarantees Secure Setup.
\end{theorem}

\paragraph*{Obtaining TAGA II.}
Then $\mcF$ guarantees
Secure Setup 

We say a AKE protocol is secure for authenticated TAGA
when it satisfies Secrecy, Key Freshness, Opposite Type, 
and Agreement on Peer, Service and Location. 

\begin{theorem}
A TAGA process $T = (P,N,M)$ guarantees Security II if the 
protocol $P$ guarantees secure AKE and Agreement on Service and
Location against active adversaries. 
\end{theorem} 

\begin{figure}
\input{figures/prot-fhmqv}
\caption{\label{prot:fmqv} TAGA pairing based on the FMQV-CSL protocol}
\end{figure}

\subsection{Concrete Design}
It is straightforward to obtain a protocol that 
guarantees the required properties.
We only need to choose an AKE protocol that satisfies the
required standard secrecy and authentication properties and extend it so
that it also guarantees Agreement on Service and Location.
Our protocol of choice is the \emph{Fully Hashed
Menezes-Qu-Vanstone protocol (FHMQV) with key confirmation}
\cite{sarrEtAl:EuroPKI09,sarrEtAl:africacrypt16}. For TAGA we simply
include service and location into the key confirmation step, yielding
\emph{FMQV-CLS}. The protocol is shown in Fig.~\ref{prot:fmqv}; a detailed
explanation can be found in App.~\ref{app:fmqv}.

\begin{theorem}
Given any type of mobile unit $U$, $($FHMQV-CLS$, U, \{\})$ is a secure
authenticated LAKE process.
\end{theorem}

FHMQV is one of the strongest protocols regarding security and efficiency.
In particular, it comes with several advanced resilience properties
that, as we will see, are essential to obtain the resilience goals
required for TAGA.




==> auth-2/auth-secure-save.tex <==

\subsection{Concept and Security}
We say a TAGA process $(P, N, M)$ is authenticated when 
$P$ is an authenticated KE (AKE) protocol. Since AKE protocols 
allow one to securely establish a key in the presence of active 
adversaries it seems plausible that by using a secure AKE
protocol we can obtain secure TAGA without having to rely on employing 
a authentcity of the NFC system under $M$.
that NFC system under $M$. And
also to not share the key with the GU operator.
We have to deal with the following though: without Channel Authenticity
it is not possible to obtain the synchronization/match between
the GU's and AC's NFC links and the operator's taps, and 
and hence the alignment of setting up the secure channel and the
physical connection.
and
hence, the direct match with the physical connection.

This can be solved as follows:
First, we extend protocols so that the protocol also guarantee that the 
two parties agree on their location (i.e.\ parking slot) and service. 
Second, we extend the setup process by an additional step so that
GUs (or operators) confirm to the AC that their physical setup is
complete over the channel. Since $A$ knows the
$G$ is at the same location, it can conclude the physical connection
must be with itself and not with same $A'$ of a different location.

This gives us the following notion of TAGA security:

%if we wish a
%design whose security is no longer dependent on Channel Authenticity
%do not wish to rely on channel authenticity of the channel 

\begin{definition}
Let $T$ be a TAGA process.
\item
We say $T$ guarantees \emph{Secure TAGA II} to a GU $G$ if,
whenever $G$ has a session $(S, \Gini, \Gfin, A, K)$ then 
\begin{enumerate}
\item $(K, S)$ is a secure channel between $A$ and $G$, and
\item $A$ is located at the same location (i.e.\ parking slot) as $G$.
\end{enumerate}
\item
Similarly, we say $T$ guarantees \emph{Secure TAGA II} to an AC $A$ if,
whenever $A$ has a session $(\Amid, S, G, K, c)$ then
\begin{enumerate}
\item $(K, S)$ is a secure channel between $A$ and $G$, and
\item $G$ is located at the same location (i.e.\ parking slot) as $A$.
\end{enumerate}
\item
We say $T$ guarantees \emph{Secure TAGA II} iff $T$ guarantees
Secure TAGA II to both parties, GUs and ACs.
\end{definition}

We say a TAGA process $\mcP$ is weakly secure if, whenever an 
instance of $\mcP$ has successfully been carried out between a 
GU $G$ and an AC $A$ then $G$ and $A$ share a secure channel
for service $S$ with $\AC(L) = A$

$A$ shares a secure channel for 
some service with some $G'$ at $L$, and $G$ shares 
a secure channel for service $S$ with $\AC(L)$.

an initial/mid NFC tap (in their view). We don't need
\begin{definition}
We say a TAGA process $\mcP$ is 
\end{definition}
NFC system guarantees `synchronization'.
if, whenever AC or GU initiate a TAGA session based on
initial or mid NFC tap, then there is indeed an operator who performs
an initial/mid NFC tap (in their view). We don't need 


\begin{theorem}
Let $\mcF$ be a process flow that integrates TAGA process $\mcP$,
and guarantees th TAGA requirements. If $\mcP$ is bla secure 
secure and  


Then $\mcF$ guarantees
Secure Setup 
We say a AKE protocol is secure for authenticated TAGA
when it satisfies Secrecy, Key Freshness, Opposite Type, 
and Agreement on Peer, Service and Location. 
\end{theorem}


\begin{theorem}
A TAGA process $T = (P,N,M)$ guarantees Security II if the 
protocol $P$ guarantees secure AKE and Agreement on Service and
Location against active adversaries. 
 \end{theorem} 

\begin{figure}
\input{figures/prot-fhmqv}
\caption{\label{prot:fmqv} TAGA pairing based on the FMQV-CSL protocol}
\end{figure}

It is straightforward to obtain a protocol that 
guarantees the required properties.
We only need to choose an AKE protocol that satisfies the
required standard secrecy and authentication properties and extend it so
that it also guarantees Agreement on Service and Location.
Our protocol of choice is the \emph{Fully Hashed
Menezes-Qu-Vanstone protocol (FHMQV) with key confirmation}
\cite{sarrEtAl:EuroPKI09,sarrEtAl:africacrypt16}. For TAGA we simply
include service and location into the key confirmation step, yielding
\emph{FMQV-CLS}. The protocol is shown in Fig.~\ref{prot:fmqv}; a detailed
explanation can be found in App.~\ref{app:fmqv}.

\begin{theorem}
Given any type of mobile unit $U$, $($FHMQV-CLS$, U, \{\})$ is a secure
authenticated LAKE process.
\end{theorem}

FHMQV is one of the strongest protocols regarding security and efficiency.
In particular, it comes with several advanced resilience properties
that, as we will see, are essential to obtain the resilience goals
required for TAGA.






==> auth-2/auth-secures20.tex <==

\subsection{Concept and Security}
We say a TAGA process $(P, N, M)$ is \emph{authenticated} when 
$P$ is an authenticated KE (AKE) protocol. Since AKE protocols 
allow one to securely establish a key in the presence of active 
adversaries authenticated TAGA has the advantage that we do not 
need to rely on the TAGA transport to guarantee channel authenticity. 
We have to deal with the following though: without channel authenticity
it is not possible to obtain Secure TAGA in the strong sense that
the GU's and AC's NFC ssns are provably matched with the operator's 
NFC taps. Hence, while by using an AKE protocol it is easy to establish 
secure channels between ACs and  GUs
it is a priori not clear how to ensure that the cyber channels indeed
match the physical connections. 
This concerns two aspects: the connections themselves and also 
the timing of the setup.

It turns out that the match between the cyber channels and physical connections
can also be established based on the following two conditions:
The first is that two parties that complete the AKE protocol 
always agree on the parking slot they are located at. 
This can be achieved by each party providing its location as data in
the protocol to the other.
The second condition is that a GU confirms over the established channel 
when its physical setup is complete. %This works for a simple reason:
Since the AC knows that 
$G$ is at the same location, it can thus conclude that any physical connection
$G$ has set up must be with itself and not with same $A'$ at a 
different location.

%if we wish a
%design whose security is no longer dependent on Channel Authenticity
%do not wish to rely on channel authenticity of the channel 

\begin{definition}
Let $T$ be a TAGA process.
\item
We say $T$ guarantees \emph{Secure TAGA II} to a GU $G$ if,
whenever $G$ has a session $(S, \Gini, \Gfin, A, K)$ then 
\begin{enumerate}
\item $(K, S)$ is a secure channel between $A$ and $G$, and
\item $A$ is located at the same parking slot as $G$.
\end{enumerate}
\item
Similarly, we say $T$ guarantees \emph{Secure TAGA II} to an AC $A$ if,
whenever $A$ has a session $(\Amid, S, G, K, c)$ then
\begin{enumerate}
\item $(K, S)$ is a secure channel between $A$ and $G$, and
\item $G$ is located at the same parking slot as $A$.
\end{enumerate}
\item
We say $T$ guarantees \emph{Secure TAGA II} iff $T$ guarantees
Secure TAGA II to both parties, GUs and ACs.
\end{definition}

\begin{definition}
We say a process flow $\mcF$ is \emph{well-defined} for
authenticated TAGA when the process satisfies the following
requirements (in addition to the others):
\begin{enumerate}
\item Whenever a GU has completed both its physical setup and 
the establishment of a cyber channel then the GU
will communicate that it's ready over the cyber channel.
\item The AC will not engage into the service before it had
confirmation from $n_\mcF$ GUs that they are ready.
\end{enumerate}
\end{definition}

In practice this requires that the GU control knows
when its physical setup is ready. This can be done by integrating
a `ready button' the GU operator will press on completion of the
setup. Or a signal is automatically generated when the
GU operator switches on a supply button (which is 
usually the last step in a setup process).

\begin{theorem}
\label{thm:setupAuth}
Let $\mcF$ be a process flow, and $T$ be a TAGA process such
that $\mcF$ includes $T$. If $\mcF$ is well-defined for authenticated
TAGA and $T$ guarantees Secure TAGA II then $\mcF$ guarantees Secure Setup.
\end{theorem}

To reach Secure TAGA II ACs and GUs must be able to communicate
their location. This requires that each AC and GU must have a
\emph{location input mechanism} installed that ensures that
the current parking slot is known to their TAGA controller. This
can be either manual: the GU operator, and pilot respectively,
input the number of the slot via a user interface. Or automatic:
the slot might already be available in the electronic system of
the GU, and AC respectively.
It could also be based on GPS coordinates, which would be most
independent of any infrastructures and human input. 

We require the underlying protocol to satisfy standard
properties of KE protocols such as secrecy, key freshness, and
mutual authentication, which we capture as injective agreement between the
runs of the two parties \cite{lowe:auth97}. For TAGA we also
require that this includes agreement on location and service.
Moreover, the property
`Opposite Type' reflects that entities have a fixed role in our setting.

\begin{definition}
We say a KE protocol is \emph{secure for authenticated TAGA}
when it satisfies Secrecy, Key Freshness, Opposite Type, 
and Agreement on Peer, Service and Location against active
adversaries. 
\end{definition}

\begin{theorem}
\label{thm:tagaAuth}
A TAGA process $T = (P,N,M)$ guarantees Secure TAGA II if the 
protocol $P$ is secure for authenticated TAGA and $M$ includes
a location input mechanism for ACs, and GUs respectively.
\end{theorem} 

\begin{figure}
\input{figures/prot-fhmqv}
\caption{\label{prot:fmqv} TAGA pairing based on the FMQV-CSL protocol}
\end{figure}

Fig.~\ref{prot:fmqv} shows TAGA based on the \emph{Menezes-Qu-Vanstone protocol 
(FHMQV) with key confirmation}
\cite{sarrEtAl:EuroPKI09,sarrEtAl:africacrypt16}. For TAGA we simply
include service and location into the key confirmation step, yielding
\emph{FMQV-CLS}. 
FHMQV is one of the strongest protocols 
regarding security and efficiency.
It also comes with several advanced properties
that, as we will see, are essential to obtain the resilience goals
required for TAGA.

\begin{corollary}
The TAGA process $T = ($FHMQV-CLS$, N, \{$LM-AC, LM-GU$\})$, where
$N$ is any type of NFC system, and LM-AC and LM-GU are location
input mechanisms,  guarantees Secure TAGA II.
\end{corollary}



==> auth-2/challenge-301.tex <==
\subsection{The Challenge of LTKC}

Let $A$ be an AC. We say the attacker has obtained a \emph{long-term 
key compromise (LTKC)} of $A$ if he has managed to get hold of 
credentials that authenticate $A$: a public/private key pair 
$(W_A, w_A)$ and a valid certificate $\cert(A, W_A)$, which asserts 
that $W_A$ belongs to $A$. The definition for a GU $G$ is analogous.
%We consider a LTKC to be a major IT security incidence of the
%respective airline, or airport respectively.
 
There are many different ways of how an attacker might obtain
a LTKC of a party $X$. One way is to obtain the private key of $X$
and use the existing certificate belonging to $X$. Another way is that the 
attacker tricks the certification authority (CA) into issueing a certificate 
for a key pair he has generated himself, perhaps for an entity that
does not even exist. This is more indirect but often easier to obtain; e.g.\  
when the private keys are generated within hardware security modules
and never exported
from there. Finally, if the attacker manages to get hold of the private key 
of the respective CA then he can generate as many valid certificates
for self-generated key pairs as he likes. All these cases have
been shown to be possible for real key management applications, e.g.\ by 
exploiting vulnerabilities in the APIs of the employed hardware
security modules \cite{AndersonBCS:survey,bfs:acm}.
%OR hash problems (see ...) 

Given a LTKC of an entity $X$ it is clear that the attacker can 
impersonate $X$ to other entities. In classical AKE settings this will only
impact on $X$'s resources or on peers that communicate specifically
with $X$ (based on $X$'s identity). However, in our setting of local
key establishment, 
%id-indiscriminate in that KE processes, 
a LTKC of an AC, say $A_I$, has wider consequences: 
given any GU $G$ that is to
service the AC at some parking slot $L$, the attacker can impersonate
$\AC(L)$ to $G$ using the credentials of $A_I$. 
A concrete attack is shown in App.~\ref{app:auth}.
%We illustrate this by the following concrete attack.
 
\removed{
\begin{figure}
\input{figures/att-ltkc}
\caption{\label{fig:att:ltkc}Attack~\ref{att:ltkc}: 
Impersonation to GU with LTKC of any AC}
\end{figure}

\begin{attack}[Impersonation to GU with LTKC of any AC]
\label{att:ltkc}
Let $A_I$ be a real or non-existent AC of airline $\mcA_I$, and assume
the attacker has achieved a LTKC of $A_I$. Further, let $A$ be an AC of 
airline $\mcA$, and $G$ be a GU at airport $\mcH$ such that 
$G$ provides service $S$ to $A$ during turnaround at parking slot $L$. 
%Assume TAGA pairing uses a passive NFC card as mobile unit. 
In preparation, the attacker swaps his own counterfeit card
$U_I$ for the card of $G$'s operator.
 Moreover, the attacker sets up NFC eavesdropping capability,
and his own WLAN access point $\AP_I$ within range of $L$. Both 
$\AP_I$ and $U_I$ are prepped with $A_I$'s long-term 
credentials $w_I$ and $\cert(A_I, W_I)$, 
a fixed ephemeral key pair $(r_I, R_I)$, and an ssid $\ssid_I$ for
the attacker's WLAN.  

Then the attacker can proceed as shown in Fig.~\ref{fig:att:ltkc}:
he simply establishes a key with $G$ using $A_I$'s credentials rather
than those of $A$. Since $A_I$'s  ephemeral key pair can be fixed beforehand,
the resulting session key can be computed independently on the card $U_I$,
and the attacker's WLAN point $\AP_I$ respectively. The latter only 
needs to receive 
$G$'s public keys by relay from the eavesdropping device. Altogether, 
the attacker can now mount a potentially safety-critical M2M Imp2GU
attack.
\end{attack}
}

In contrast, a LTKC of a GU $G$ does not have an equally wide impact:
Since a GU is specific to its airport, and an AC knows at which
airport it is currently parked (available from the electronic flight
system of the AC) an AC can easily validate that the airport within 
a presented GU certificate
agrees with its own location. This means a compromised GU certificate can only
be abused in the realm of its airport. 

\removed{
As shown a single remotely 
obtained LTKC at airline $\mcA$ can impact on the safety of any AC of
$\mcA$.  

Note that this violates Principle~\ref{p:localAL} `Trust in Airline of
Local AC and no Other': a LTKC at airline $\mcA_I$ can impact on the
safety of an AC of airline $\mcA$. And even when $\mcA = \mcA_I$
this violates Principle~\ref{p:localACResil} 
`Resilience against Remote AC Security Incidence': 

Hence, it is essential
to harden authenticated TAGA against LTKC. 
We now
discuss other threats posed by LTKCs in this setting, and how 
we can still achieve resilient authenticated TAGA by a combination of advanced 
properties of AKE protocols and additional process measures that
exploit the local setting.  
}

\input{auth-2/further}


\removed{
In a classical AKE setting the credentials of a user $A$ are typically
used as follows: either they govern access to resources bound to $A$ 
such as $A$'s money, data, or account on a computing system; or 
they establish $A$'s identity to peers that wish to communicate with
$A$ (and $A$ specifically). Given a LTKC of $A$ it is clear that the 
attacker can impersonate $A$. However, this will only impact on $A$'s 
resources or on peers that communicate with $A$ based on its identity.

In our setting the credentials of an AC $A$ are used in a different
way: they give access to establishing a secure channel with any GU 
at any airport that takes part in TAGA. This is so because
a priori the GU, say $G$, does not know the identity of $A/AC(L)$ but 
establishes the channel with any AC that has valid credentials 
and says they are at the same location as $G$. Hence, a LTKC of $A$
has wider consequences here: given any GU $G$ that is dispatched to service
an AC at location $L$, the intruder can impersonate $\AC(L)$ to $G$. 
Moreover, the attacker has the power to affect the safety of
this AC. as discusse din Section~\ref{} can be safety-critical. 
}



==> auth-2/further.tex <==

\paragraph*{Futher}
However, in general it is not the case that ltkc only imp 
whiel one cannot avoid (on protocol level) that ltcs allows
x and ltkc allows y. the other direction doesn't hold. 
if the protocol does not guarantee certain resilience.
it is instructive to have som exmples. e.g.

\begin{definition}
Let $P$ be a protocol that is secure for ATAGA. We say $P$ guarantees 
to an AC $A$ LTKC resilience if $P$
guarantees the secrecy and authentication properties to $A$ even
when $A$ has a LTKC.  
The definition for a GU $G$ is symmtric. We say $P$ guarantees
LTKC resilience if $P$ guarantees this to all parties.
\end{definition}

\begin{lemma}
Let $P$ be a protocol that is secure and LTKC resilient for ATAGA.
Assuming that system integrity of GUs, ACs is given (including that
ephemeral keys are secure (not required).
\begin{enumerate}
\item If $G$ has a session $(S, A, K)$ and the attacker knows $K$
      then $A$ has a LTKC. hence some AC. 
\item If $A$ has a session $(S, G, K, ..)$ and the attacker knows
 $K$ then $G$ has a LTKC. hence by checks GU ..
\end{enumerate}
assuming no other incidences apart from LTKCs
\end{lemma}

if all keys are secure secrecy is given. so must be ..


==> auth-2/variants.tex <==

NFC system guarantees `synchronization'.
if, whenever AC or GU initiate a TAGA session based on
initial or mid NFC tap, then there is indeed an operator who performs
an initial/mid NFC tap (in their view). We don't need



==> plain-2/attacks-save.tex <==

\subsection{The Challenge of Channel Authenticity}
We now illlustrate that it is rather challenging to obtain
channel authenticity. Even though TAGA takes place in a secure
zone, where only authorized personnel have access, it turns out 
that the attacker has various indirect ways of compromising the 
TAGA transport. 

\paragraph*{Swapping the TAGA Card}
During a break a GU operator might reside in a less restricted area. 
An attacker with pickpocketing capability could  
use this as a window of opportunity to swap the TAGA card (carried by
the operator throughout the day) with a counterfeit card he has 
prepared himself. Since pickpocketing can include social engineering 
such a card swap 
cannot be ruled out entirely even when the card must be worn physically 
attached to the operator,
e.g.\ by a lanyard\footnote{A lanyard is a cord or strap worn around 
the neck or wrist for security.}.

\paragraph*{Eavesdropping}
Another threat is that the attacker eavesdrops on the NFC exchange 
between the card and the GU or AC reader. While the nominal range 
of NFC communication is about 10 cm  5-10 cm.
it has been shown that the range of eavesdropping can be  
considerably increased. Finke and Kelter \cite{FK:05} first 
demonstrate that the communciation between a ISO-14443 reader 
and tag can be eavesdropped from 1-2 meters using a large loop
antenna. As reported in \cite{HasBr:RFID06} eavesdropping on a device
that is sending in active mode (like the GU and AC reader)
has a range of about 10 m. Moreover, \cite{Kfir:2005} 
show a distance of tens of meters when an active antenna is used 
by simulation. A large antenna could be hidden in large luggage, sports 
equipment, prams or wheelchairs, cages for pets, instruments etc. 
Maybe even in clothing of operators such as a safety vest that was 
swapped beforehand. Hence, it seems impossible that eavesdropping
can be ruled out by practically enforceable measures.

A small antenna (with less range but relay functionality) 
could be smuggled into the pockets 
of the operator,
or hidden in his clothing such as a safety vest that was swapped
beforehand. 

\paragraph*{Leech Attacks and Skimming (against a card)}
In the context of relay attacks against electronic payment systems
it is common that the attacker makes use of a ``leech'' device.
The leech device can e.g. be smuggled into a victims pocket 
or bag so that it is close to their payment card. There the leech can
power the tag of the card, communicate with it, and relay the communication
to and from a reader via his laptop (e.g. by WLAN). A leech can
also be employed as a skimmer to read out a tag (without writing to
it). It has also been shown that by increasing the power of transmission
and/or using larger antenna a leech device can increase its
range beyond the nominal range. \cite{Kfir:2005} predicated a distance of
40-50 cm by simulation, \cite{KirWool:UsenixSec06} have experimentally shown
a skimming range of 25 cm. % and \cite{} skimming. 

Similarly to card swapping an attacker could easily smuggle 
a leech device into an operators pocket. Moreover, a particular threat in 
our setting is that a standard device with NFC capability such as 
the smartphone of an operator is converted into a leech by malware. 
We call such a leech `software-leech'. 
 
\paragraph*{Ghost Attacks (against a reader)}  
Another threat in our setting is that an attacker's ghost device
communicates with one of the readers pretending to be a TAGA card.
At first this seems impossible in the setting of TAGA where
only authorized personnel have access close to the readers:
to present a fake card to a TAGA reader an attacker needs to
be within acivation range, i.e. within the ....
However, an attacker can use an \emph{active} ghost "to increase
the distance from which the ghost can receive the reader's signal.
This is possible because the ghost can "ignore any
regulatory limitations and does not use the standard load modulation.
As shown in \cite{Kfir:2005} by simulation
the ghost can be about 50m away fromt the reader. 
based on modeling and simulations
Hence, a ghost could even be remote or it could come as a device 
infilatrated into the GU or onto an operator. be implemented

While this seems impossible at first sight due to the fact 
an be done from remote or from an infiltrated device.

\subsubsection{Examples}
Now show examples how this can be combined to carry out
mitm attacks against a naive implement. of plain taga.
They are all variations of the well-known ..DH ...


\removed{
can be clearly formulated and realistically enforced is that he 
can eavesdrop on the NFC exchange between the card and the
TAGA controller (on either side). formula passive NFC. 
While it seems not easy for a practical attacker to do this,
there are many options: camouflage the antenna in bulky luggage 
(e.g. as a movable trampolin, surfboard), sth attached to the
operator herself (by social eningeering or swap of work jacket).
And not sufficient data available to rule out by a clear argument, 
perhaps because usually in secure applicaiton this is not necessary.
difficult to rule it out .}

\paragraph*{MitM despite Passive NFC Card}
The following attack shows that the combination of
eavesdropping and card swapping is all the attacker needs to
obtain full MitM capability. 

%Altogether, this means the following MitM attack is possible.

\begin{figure}
\vspace{3cm}
\caption{\label{fig:att:swap} Attack~\ref{att:swap}}
\end{figure}

\begin{attack}[MitM by Swap \& Eavesdrop]
\label{att:swap}
Let $A$ be an AC and $G$ be a GU at parking slot $L$ so that
$G$ is to service $A$. In preparation, the attacker swaps
the card of $G$'s operator with his own prepared card $U_I$
as described above. Moreover, the attacker sets up NFC
eavesdropping capability, and his own WLAN access point $\AP_I$
in the range of $L$. Both $U_I$ and $\AP_I$ are prepped with
a fixed ephemeral key $(r_I, R_I)$, and an ssid $\ssid_I$ 
for the attacker's WLAN. 

Then the attacker can carry out the classic MitM attack against
the DH exchange as depicted in Fig.~\ref{fig:att:swap}. With the
second NFC tap the counterfeit card writes the attacker's public key 
$R_I$ to $A$ rather than $G$'s public key $R_G$. And similarly, with
the third NFC tap the card writes $R_I$ and $\ssid_I$ to $G$ rather 
than $A$'s public key $R_A$ and ssid $\ssid_A$. Hence, $G$ will
compute session key $K_\GI$ based on $r_G$ and $R_I$, and
$A$ will compute  session key $K_\IA$ based on $r_A$ and $R_I$.

To be able to set up the corresponding ``secure'' channels with
$G$, and $A$ respectively, the attacker must somehow get 
$R_G$ and $R_A$ to his WiFi point $\AP_I$. Since the card only has 
a passive NFC interface  this information cannot be forwarded directly 
from the card. Instead, the attacker 
obtains $R_G$ and $R_A$ by eavesdropping on the first, and respectively
second, NFC tap, and relays the information from the respective
eavesdropping device to $\AP_I$.
There the attacker will compute the key $K_\GI$ he shares with $G$, 
and the key $K_\IA$ he shares
with $A$, and establish the corresponding channels.
% with $G$, and
%that with $A$ respectively.
\end{attack}

If the attacker has difficulties in
setting up eavesdropping capability he could also 
skim the public keys by a leech device. 
The leech could be planted on the operator at the same
time as the card swapped, e.g. in a classical `pour drink over
shirt' attack.

\removed{
In practice, it might be challenging to set up
the eavesdropping cabability. However, because we are aiming for
designs that can be shown to be provably secure it is difficult
to exclude eavesdropping. The next attack is realistic, and 
includes an alternative way to eavesdropping.
to relay information from a passive NFC 
card to an attacker's server. Moreover, this attack works with
an authentic TAGA card. no swap 
The technique of a hacked smartphone below 
This attack is }

\subsubsection{MitM with Hacked Smartphone}
During the TAGA transport the operator might carry a smartphone
with NFC capability with him. 
%We assume the smartphone is equipped with an active
%NFC element. 
An attacker with standard hacking capability could 
compromise the smartphone, e.g.\ by planting malware on the
device via a Trojan app or a spear phishing email to the operator. 
Then, if the operator stores the smartphone close enough to the NFC card 
during the TAGA transport the compromised phone can read from and write to the 
card. On the one hand, this gives the attacker means to relay 
information to/from his own WiFi station outside the secure zone
(E.g.\ in Attack~\ref{att:swap} the public keys of the GU and AC 
could be read out and relayed as an alternative to eavesdropping 
them.) On the other hand, this  might
allow him to carry out a MitM attack without having to break integrity or 
authenticity of the card: the phone can
masquerade as the TAGA controller of the AC, and GU respectively,
and thereby overwrite the public keys of the GU and AC 
with his own key.

We have implemented this attack against the current prototypical
implementation of TAGA. It works whenever the GU operator is in 
the habit of carrying a smartphone in his pocket, and storing the 
TAGA card in the same pocket next to the smartphone while he walks 
from the GU to the AC, and similarly for the way back. This is a 
natural assumption: the operator typically needs both hands to 
carry the supply hose and might not like the dangling of a lanyard.

\begin{figure}
\vspace{3cm}
\caption{\label{fig:att:phone} Attack~\ref{att:phone}}
\end{figure}

\begin{attack}[MitM with Hacked Smartphone]
\label{att:phone}
Let $A$ be an AC and $G$ be a GU at parking position $L$ so
that $G$ is to service $A$. In preparation, the attacker 
hacks the smartphone of the operator of $G$, say $P_I$, and sets up
his WiFi point $\AP_I$ in the range of $L$. The attack proceeds
as shown in Fig.~\ref{fig:att:phone}. We assume that the
TAGA card is a simple store NFC card with a register Reg1 assigned
for the first message, and a register Reg2 for the second. 

The first NFC tap proceeds as usual, and writes $G$'s message 
into register Reg1 of the card. After the tap the
operator puts the card into his pocket next to his hacked
phone $P_I$. This triggers the NFC module of $P_I$, upon which it
reads the contents of Reg1 (i.e.\ $G$'s public key) and then 
overwrites them with his own key $R_I$. 
Hence, when the operator arrives
at the AC and performs the (supposedly) second NFC tap
the AC reads the attacker's key $R_I$. The second message
pass is manipulated in the analogous fashion. The attacker
can easily relay the public key of $G$, and $A$ respectively,
from the hacked smartphone to his access point $\AP_I$.
Now he can establish keys and WiFi sessions with both 
$G$ and $A$, and act as man-in-the-middle.
\end{attack}

\removed{
The technical details of the proof-of-concept implementation
can be found in App.~\ref{app:attack}. The attack works reliably as 
long as the operator observes his habit of storing the card in
his pocket next to the phone.}

If a more complex card than a simple store card is employed 
Attack~\ref{att:phone} can be
prevented by keeping state of the taps, and implementing
an input/output check. However, such
measures can easily be overcome by carrying out a multi-session attack
instead.

\begin{attack}[Multi-session Variation]
When the phone first interacts with the card it will now 
perform three read/writes instead of one: the first impersonates
the AC and reads $G$'s public key; the second impersonates the GU 
during the final tap and concludes the current session of the card; 
the third read/write starts a fresh session, it impersonates the GU 
and writes the attackers key $R_I$.
The next tap will be carried out with the real AC in the appropriate
state, but of a new session, which is unnoticeable for the AC.
On the way back the attacker can proceed in the analogous fashion.
\end{attack}

\subsubsection{Impersonation from Remote./Ghost}
Unfortunately it also seems possible to actively talk to a TAGA reader
from about 50 m. CHECK Then Imp2AC is possible from a distance. 
In our services there is not safety impact. But of course there might
be others. This violates Principle Local Connection.

"ghost is a device which fakes a card to the reader"

present the ghost to the reader at paytime. 
leech to operator during break, relay this to someone.

Since TAGA employes a passive smartcard, one would expect that
to masquerade as a regular TAGA card an attacker's device has
to success.present a fake card to a TAGA reader an attacker would have
to be within ``activation range'', i.e.  within the secure zone. 


the active readers  

\removed{
\subsubsection{Full Dependency on GU Operator}
One assume card cannot be swapped and bound to the GU.
While the GU Operator is a trust anchor in ..
The following shows that by using two cards he can always
undermine the process.
he can do this fully covertly in his pocket. even when
under camera surveillance.
}


==> plain-2/concl.tex <==

\subsection{Discussion and Resilience}

This shows how to obtain secure plain TAGA./indeed possible.
To sum up, while the zone of a turnaround leaves open many
indirect attacks against the TAGA channel we can still obtain
plain TAGA:
we can bootstrap channel authenticity from binding the card to
the GU and guaranteeing a secure proximate zone around the readers.

However, there are two drawbacks. One is that the status of
distance bounding of real NfC systems is still not mature
(c.f.\  ). bla discuss problems. 
This could be solved in the meantime by reverting to normal
card reading system. (The proofs carry through. Proximate assumptions
come for free.)

The other drawback is principal though: the security
depends on the operator. While the operator is a trust anchor
from the viewpoint of safety,
from viewpoint of secure key establishment it seems unorthodox
to make them the trusted  it is unorthodox from the
perspective of secure key establishment of making him essentially
a trusted third party who can obtain the key with little effort.

\paragraph*{Resilience}

\paragraph*{other}
The limitation of plain TAGA is that security depends on 
Operator following ... One could even claim that the
usual Secrecy guarantee requirement of a session key is not fulfilled:
if one includes a model of the op with basic abilities and only
covert actions then a mitm is always possible.

Hence, liability, also extension id not bound to .

tension betwen practic and provability

e.g. requirments: need to practically enforcable..

unlikely no luggage but requ: there should be no 

and what is the probability?


==> plain-2/conds-op.tex <==
\subsection{Authenticity of TAGA Transport}
only one device matches tap
gini = DH session msg agree

$<$ earlier than

From Assumption:
Then obtain: if $\nfcl{s1}{s2}$ then $\msg(s_1) = \msg(s_2)$


\begin{enumerate}
\item GU and AC readers guarantee proximity of $\partner(link)$.
\item $M$ guarantees that any device proximate to a GU or AC
    reader is a card carried by an OP.
\item OP only bring a card proximate to a GU or AC reader on a regular
TAGA walk.
\item TAGA walk satisfies certain conditions.
\end{enumerate}



\begin{definition}[Guarantees to GU]
Let $N$ be a NFC system.
\item
We say $N$ guarantees \emph{`authenticity of initial tap to a GU $G$'} if,
whenever $G$ has a session $(S, \Gini, \ldots)$ 
then there is an \emph{authentic} card $C$ with a session 
$(\Cini, \ldots)$ such that 
\begin{enumerate}
\item $\nfcl{\Gini}{\Cini}$ and $\msg(\Gini) = \msg(\Cini)$, and
\item $C$ is proximate to $G$ during $\Cini$.
\end{enumerate}
\item
We say $N$ guarantees \emph{`authenticity of final tap to a GU $G$'} if,
whenever $G$ has a session $(S, \Gini, \Gfin, \ldots)$ and `authenticity
of initial tap' is guaranteed to $G$ then there is an authentic card 
$C$ with a session $(\Cini, \Cmid, \Cfin)$ such that 
\begin{enumerate}
\item $\nfcl{\Gini}{\Cini}$, 
\item $\nfcl{\Gfin}{\Cfin}$ and $\msg(\Gfin) = \msg(\Cfin)$, and
\item $C$ is proximate to $G$ during $\Cfin$.   
\end{enumerate}
\end{definition}

\begin{definition}[Guarantees to Card]
Let $N$ be a NFC system.
\item
We say $N$ guarantees
\emph{`integrity of a $N$ card $C$'} if, whenever $C$ has a session
$(\Cini, \Cmid, \Cfin)$ then 
\begin{enumerate}
\item $\msgr(\Cini) = \msgs(\Cmid)$, and
\item $\msgr(\Cmid) = \msgs(\Cfin)$. 
\end{enumerate}
And similarly for partial sessions.
\item
We say $N$ guarantees
\emph{`authenticity of initial tap to a $N$ card $C$'} if, whenever $C$
has a session $(\Cini, \ldots)$ then there is some GU $G$ with
a session $(S, \Gini, \ldots)$ such hat 
\begin{enumerate}
\item $\nfcl{\Cini}{\Gini}$, and $\msg(\Cini) = \msg(\Gini)$, and
\item $C$ is proximate to $G$ during $\Cini$.
\end{enumerate}
\item
We say $N$ guarantees
\emph{`authenticity of mid tap with AC to a $N$ card $C$} if, whenever
$C$ has a session $(\Cini, \Cmid, \ldots)$ and $\partner(\Cmid)$ is
an AC $A$ then $A$ has a session $(\Amid, \ldots)$ such that
$\nfcl{\Cmid}{\Amid}$ and $\msg(\Cmid) = \msg(Amid)$. 
\removed{
\item
We say $N$ guarantees
\emph{`authenticity of final tap to a $N$ card $C$'} if, whenever
$C$ has a session $(\Cini, \Cmid, \Cfin)$ and `authenticity
of initial tap' is guaranteed to $C$ then there is some GU $G$ 
with a session $(S,\Gini,\Gfin, \ldots)$ such that 
\begin{enumerate}
\item $\nfcl{\Cini}{\Gini}$, 
\item $\nfcl{\Cfin}{\Gfin}$ and $\msgs(\Cfin) = \msgr(Gfin)$
\end{enumerate}
}
\end{definition}

\begin{definition}[Guarantees to AC]
Let $N$ be an NFC system.
\item
We say $N$ guarantees \emph{`proximity of NFC peer to an AC $A$'} if,
whenever an AC $A$ has a session $(\Amid, \ldots)$ 
then $\partner(\Amid)$ is proximate to $A$ during the NFC ssn.
\item
We say $N$ guarantees \emph{`authenticity of mid tap with an authentic 
card to an AC $A$'}, if
whenever $A$ has a session $(\Amid, \ldots)$ and $\partner(\Amid)$
is an authentic card $C$ then $C$ has a session 
$(\Cini, \Cmid, \ldots)$ such that 
$\nfcl{\Amid}{\Cmid}$ and $\msg(\Amid) = \msg(\Cmid)$.
\end{definition}

\begin{proposition}
\label{prop:nfc}
\item
\begin{enumerate}
\item
If a GU or AC reader $R$ has a NFC ssn $\Rx$ and $\partner(\Rx)$ is 
proximate during $\Rx$ then there is an operator tap $\Wx$ such that
\begin{enumerate}
\item $\card(\Wx) = \partner(\Rx)$, and
\item $\tapl{\Wx}{\Rx}$.
\end{enumerate}
\item
If there is an operator tap $\Wx$ and $\reader(\Wx)$ is a GU or
AC reader $R$ then $R$ has a NFC ssn $\Rx$ such that
\begin{enumerate}
\item $\card(\Wx) = \partner(\Rx)$, and
\item $\tapl{\Wx}{\Rx}$.
\item If $R$ is a GU reader then $C$ is authentic.
\end{enumerate}
\end{enumerate}
\end{proposition}

\begin{proof}
(1)~This follows from `secure proximate zone'.

(2)~Since the operator visually verifies that the reader has 
successfully completed an NFC exchange (e.g.~green light) $\Rx$ exists.
By `secure proximate zone' the exchange must have indeed been carried
out with the operator's card. If the reader is a GU the GU will
check authenticity of the card during the exchange, and the
NFC exchange will fail if it is not (e.g.~red light). 
\end{proof}

\paragraph*{Operator}

\begin{fact}[Operator session]
\label{fact:walk}
For every operator session $(\Wini, \Wmid, \ldots)$ we have:
\begin{enumerate}
\item $\reader(\Wini)$ is a GU $G$,
\item $\reader(\Wmid)$ is an AC $A$,
\item the location of $G$ and $A$ is the same,
\item $\card(\Wini) = \card(\Wmid)$,
\item There are no taps with $C$ to $G$ between $\Wini$ and
      $\Wmid$. OP goes straight to A
\end{enumerate}
\end{fact}

\begin{proof}
This is a consequence of how the TAGA pairing process is defined.
\end{proof}

  i.e.\ presses abort button after display information.

\begin{enumerate}
\item When an operator performs a tap $\Wx$ with the reader of a
GU $G$ and $G$'s reader displays that a new TAGA session is initialized then 
either the operator is on a TAGA walk/has a TAGA session $(\Wx, \ldots)$
or he will abort $G$'s session before carrying out any further taps with $G$.

\item When an operator is on a TAGA walk/session $(\Wini, \ldots)$ 
and carries out the mid tap with the reader of an AC $A$ then either
the tap is successful (e.g.\ green light) or the operator aborts 
the session of $\reader(\Wini)$ before carrying out any further
taps with that GU.

\item An operator taps an AC only as part of the mid tap of a TAGA session.
\end{enumerate} 

Taps only as part of TAGA sessions:

\begin{enumerate}
\item If there is an operator tap $\Wx$ such that 
  $\reader(\Wx)$ is a GU $G$, $\tapl{Wx}{\Gini}$ for a GU session
  $(S, \Gini, \ldots)$ then the operator has carried out the
  tap indeed as part of a session
  $(\Wx, \ldots)$ or immediately aborts the GU session 

\item When there is an operator tap $\Wac$ at the reader of AC $A$,
   and $A$ reports back `successful mid TAGA tap' then the operator
   has a TAGA session $(\Wini, \Wac, \ldots)$. If $A$ reports
   back something else the operator will abort the session at
   $\reader(\Wini)$ before any further taps.

\item If OP has started a session $(\Wini, ..)$ then the next tap is
  with AC at $L$/ then he either completes it to a $(\Wini, \Wmid, \Wfin)$
   or aborts the GU session before any further taps. 
\end{enumerate}

\begin{fact}[Taps and operator sessions]
\label{fact:tapsWalk}
\item
\begin{enumerate}
\item If there are operator taps $\Wx$ and $\Wy$ and a GU
      session $(S, \Gini, \Gfin, \ldots)$ such that
      $\tapl{\Wx}{\Gini}$ and $\tapl{\Wy}{\Gfin}$ then
      there must be an operator session $(\Wx, \Wmid, \Wy)$ for
      some $\Wmid$.

\item If there is an operator tap $\Wac$ and an AC session 
      $(\Amid, \ldots)$ such that $\tapl{\Wac}{\Amid}$ then 
      there must be an operator session 
      $(\Wini, \Wac, \ldots)$ for some $\Wini$.
\end{enumerate}
\end{fact}

\begin{proof}
(1) By (1) the operator will immediately abort the GU session if $\Wx$
wasn't the first tap of a TAGA session $(\Wx, \ldots)$. Since $G$
receives the last NFC ssn the latter must be true. 
By WALK the operator will carry on to the AC. By (2) the tap is
either successful or the operator will immediately abort 
$G$'s session. Since $G$ receives the last NFC ssn the former must
be true. But then $\Wmid$ exists as required. 

(2) This follows by (3).
\end{proof}

\begin{proof}
(1) $\Gini$ initiates an OP session $(\Wx, \ldots)$.
Since $\Gfin$ the operator has not aborted the session. Then
the OP has completed a walk $(\Wini, \Wmid, \Wfin)$. 
with one $C$ at most one comm, must have happened with $\Wmid$.
only one tap.
\end{proof}

\begin{fact}[Operator session]
\label{fact:walk}
Given an operator session $(\Wini, \Wmid, \ldots)$ we have:
\begin{enumerate}
\item $\reader(\Wini)$ is a GU $G$,
\item $\reader(\Wmid)$ is a AC $A$,
\item the location of $G$ and $A$ is the same,
\item $\card(\Wini) = \card(\Wmid)$,
\item There are no taps with $C$ to $G$ between $\Wini$ and
      $\Wmid$.
\end{enumerate}
\end{fact}

\begin{theorem}
If a NFC system satisfies ... then it guarantees Authenticity.
\end{theorem}

\begin{proof}[Proof of Authenticity]
\emph{Guarantee for GU:}
Assume $G$ has a session $(S, \Gini, \Gfin, \ldots)$ at $L$. Then
by `authenticity of initial and final tap to $G$' there is an
\emph{authentic} card $C$ with a session $(\Cini, \Cmid, \Cfin)$
such that the NFC ssns and exchanged messages are matching, i.e.: 
$\nfcl{\Gini}{\Cini}$, $\nfcl{\Gfin}{\Cfin}$, $\msg(\Gini) = \msg(\Cini)$, 
and $\msg(\Gfin) = \msg(\Cfin)$. Moreover, $C$ is proximate to $G$ 
during $\Cini$ and $\Cfin$.

By Prop.~\ref{prop:nfc}(1) there are operator taps $\Wini$, $\Wfin$
such that $\card(\Wini) = C$ and $\tapl{\Wini}{\Gini}$, and
$\card(\Wfin) = C$ and $\tapl{\Wfin}{\Gfin}$ respectively. Then by
Fact~\ref{fact:tapsWalk}(1) there is an operator with a session 
$(\Wini, \Wmid, \Wfin)$ for some $\Wmid$.

Further, by Fact~\ref{fact:walk} we obtain $\reader(\Wmid) = \AC(L)$ 
and $\card(\Wmid) = C$. Hence, by Prop~\ref{prop:nfc}(2) $\AC(L)$, 
say $A$, has 
a NFC ssn $\Aac$ such that $\partner(\Aac) = C$ and $\tapl{\Wmid}{\Aac}$.
Let $\Cac$ be defined by $\nfcl{\Aac}{\Cac}$. 
$\Cac$ takes place after $\Gini$ (and hence $\Cini$) and before $\Gfin$ 
(and hence $\Cfin$). Hence, we conclude that $\Cac = \Cmid$.
Then by `authenticity of mid tap with AC to $C$' $A$ must have
a session $(\Amid, \ldots)$ and  $\msg(\Amid) = \msg(\Cmid)$. 
Finally, by `integrity of $C$' it is straightforward to check that
the messages of the $A$ session match those of the $G$ session.

\emph{Guarantee for AC:}
Assume $A$ at $L$ has a session $(\Amid, \ldots)$. Then by
`proximity of NFC peer to $A$' $\partner(\Amid)$, say $C$, is proximate.
Then by Prop.~\ref{prop:nfc}(1) there is an operator tap $\Wac$
such that $\tapl{\Wac}{\Amid}$ and $\card(\Wac) = C$.
Then by Fact~\ref{fact:tapsWalk}(2) there is an operator with
session $(\Winiac, \Wac, \ldots)$ for some $\Winiac$. By Fact~\ref{fact:walk}
$\reader(\Winiac)$ is a GU $\Gac$ at $L$, and $\card(\Winiac) = C$.

By Prop.~\ref{prop:nfc}(2) $\Gac$ has a NFC ssn $\Giniac$ such that
$\partner(\Giniac) = C$, $\tapl{\Winiac}{\Giniac}$, and $C$ is authentic.
Let $\Ciniac$ be defined by $\nfcl{\Giniac}{\Ciniac}$.

Since $C$ is authentic by `authenticity of mid tap with authentic
card to $A$' $C$ has a session $(\Cini, \Cmid, \ldots)$ such 
that $\nfcl{\Amid}{\Cmid}$ and $\msg(\Amid) = \msg(\Cmid)$.
By `authenticity of first tap to $C$' there is some GU $G$ with a session 
$(S, \Gini, \ldots)$ such that $\nfcl{\Gini}{\Cini}$,
$\msg(\Gini) = \msg(\Cini)$, and $C$ is proximate to $G$ during
$\Cini$. By `integrity of $C$' we also obtain that the messages of $\Amid$ and 
$\Gini$ are matching. 

Moreover, by Prop.~\ref{prop:nfc}(1) there is an operator
tap $\Wini$ such that $\card(\Wini) = C$ and $\tapl{\Wini}{\Gini}$.
Hence, it only remains to show that $\Wini = \Winiac$. 
To the contrary assume this not to be the case.
Then by Fact~\ref{fact:walk}(5) $\Wini < \Winiac$, and hence 
$\Cini < \Ciniac$. But this leads to a contradication:
since $\tapl{\Wac}{\Cmid}$ and $\Cini$ immediately precedes
$\Cmid$ on $C$, we must have $\Ciniac < \Cini$.
\end{proof}



==> plain-2/conds-save.tex <==
\subsection{Authenticity of TAGA Transport}
only one device matches tap
gini = DH session msg agree

\begin{definition}[to GU]
We say $N$ gurantees
\emph{Authenticity of initial tap to a GU $G$} if, whenever $G$
has a session $(S, \Gini, ?, ?)$ then there is an authentic card $C$ 
with a session $(\Cini, \ldots)$ such that 
\begin{enumerate}
\item $\Gini = \Cini$ and $\msg(\Gini) = \msg(\Cini)$, and
\item $C$ is proximate during the NFC comm. OR: $C$ is the $G$ card. 
\end{enumerate}
\item
We say $N$ guarantees \emph{Authenticity of final tap to a GU $G$} if,
whenever $G$ has a session $(S, \Gini, \Gfin, ?)$ and Authenticity
of initial tap is guaranted to $G$ then there is an
authentic card $C$ with a session $(\Cini, \Cmid, \Cfin)$ such
that 
\begin{enumerate}
\item $\Gini = \Cini$, 
\item $\Gfin = \Cfin$ and $\msg(\Gfin) = \msg(\Cfin)$, 
\item and $C$ is proximate during the NFC comm.
\end{enumerate}
\end{definition}

\begin{definition}[to C]
We say $N$ guarantees
\emph{Integrity of a $N$ card $C$} if, whenever $C$ has a session
$(\Cini, \Cmid, \Cfin)$ then 
\begin{enumerate}
\item $\msgr(\Cini) = \msgs(\Cmid)$, and
\item $\msgr(\Cmid) = \msgs(\Cfin)$. 
\end{enumerate}
And similarly for partial sessions.
\item
We say $N$ guarantees
\emph{Authenticity of initial tap to a $N$ card $C$} if, whenever $C$
has a session $(\Cini, ?, ?)$ then there is some GU $G$ with
a session $(S, \Gini, ?, ?)$ such hat 
\begin{enumerate}
\item $\Cini = \Gini$, and $\msg(\Cini) = \msg(\Gini)$, and
\item $C$ is proximate to $G$ during the NFC comm. OR: $C$ is the $G$ card.
\end{enumerate}
\item
We say $N$ under $M$ guarantees
\emph{Authenticity of middle tap to a $N$ card $C$} if, whenever
$C$ has a session $\Cini, \Cmid, ?)$ then there is some AC $A$
with a session $(\Amid, ?, ?, ?)$ such that
\begin{enumerate}
\item $\Cmid = \Amid$ and $\msg(\Cmid) = \msg(Amid)$, and
\item $C$ is proximate to A/is $AC(L)$?? 
\item 
\end{enumerate}
\item
We say $N$ guarantees
\emph{Authenticity of final tap to a $N$ card $C$} if, whenever
$C$ has a session $(\Cini, \Cmid, \Cfin)$ and Authenticity
of initial tap is guaranteed to $C$ then there is some GU $G$ 
with a session $(S,\Gini,\Gfin, ?)$ such that 
\begin{enumerate}
\item $\Cini = \Gini$, 
\item $\Cfin = \Cfin$ and $\msgs(\Cfin) = \msgr(Gfin)$,
 and $C$ is proximate to $G$ during the NFC comm.
\end{enumerate}
\end{definition}

\begin{definition}[Guarantees to AC]
We say $N$ guarantees \emph{Proximity of NFC comm tap to an AC $A$} if,
whenever $A$ has a session $(\Amid, \ldots)$ then there is a
NFC device $D$ such that
\begin{enumerate}
\item $D$ has a matching NFC session Dtap and $\Amid = Dtap$,
\item $D$ is proximite to $A$.
\end{enumerate}
\end{definition}

\begin{definition}[Proximate NFC Exchange]
We say $N$ under $M$ guarantees \emph{Origin Authenticity of
Proximate NFC Exchange}
to an AC $A$, if
whenever an AC $A$ has an NFC exchange $Ax$ and $partner(Ax) = C$
is proximate then there is an OP $O$ with a NFC tap $Wx$ such that 
and only one.
\begin{enumerate}
\item $card(Wx) = C$ and $Wx t= Cx$.
\end{enumerate}
The definition to a GU $G$ is analogous.

session $(\Amid, \ldots)$ and
there is an NFC device $C$ with an NFC session $Cx$ such that 
$\Amid = Cx$, 
shares a NFC session with a proximate device $C$
then there is an OP $O$ with a session $(\Wini, \Wmid, \ldots)$ 
such that $\card(\Wini) = \card(Wmid) = C$.

has there is a proximate tap with D then there is an OP $O$ with
a session $(\Wini, \Wmid, ...)$ and $card(\Wmid) = D$ and 
$reader(\Wini) = G$ for some $G$ at $L$.
\item
Whenever GU has a proximate NFC comm with some $D$ then there
is an OP $O$ with a session  $(\Wini)$ or $'''$ first or second and /one
\end{definition}



\begin{definition}[to A]
\item
Auth of mid tap to $A$:
whenever $A$ has a session $(\Amid, \ldots)$ and $\Amid$ comm
partner is an authentic card $C$ then $C$ has a session
$(\Cini, \Cmid, \ldots)$ such that $\Amid = \Cmid$ and messages
agree.
\end{definition}

\begin{fact}
Whenever a GU $G$ and an authentic card $C$ have matching sessions 
then there is an OP $O$ with a session $(\Wini, \Wmid, \Wfin)$
such that $O$ taps are observ. matching (in time) $\Cini = \Gini$
\begin{enumerate}
\item $\Wini$ obs. matches $\Cini = \Gini$ tap, and 
\item $\Wfin$ obs. matches $\Cfin = \Gfin$ tap.
\item if Wini with a GU at L then Wmid with $\AC(L)$.
\end{enumerate}
\end{fact}

\begin{definition}
(ACtap)
If an OP successfully performs a tap with authentic card $C$ with an AC 
$A$ then $C$ has a session $(\Cini, \Cmid, ?)$ and $A$ has a session
$(\Amid, ...)$ such that
\begin{enumerate}
\item $\Cmid = \Amid$ and $\msg(\Cmid) = \msg(\Amid)$.

If AC has 
\end{enumerate}

\end{definition}

only a OP can be proximate to a GU.

\begin{definition}
whenever there is a tap between a GU $G$ and an authentic card $C$ 
the card is proximate to 
there is an OP who  

\end{definition}

if there is a obs. match with A and C then
there OP observes match with A/C 

\begin{definition}[to C by op]
Whenever $C$ has a session $(\Cini, \Cmid, ?)$ then there
is an OP $O$ with a session $(\Wini, \Wmid, ?)$ such that
\begin{enumerate}
\item $\Wini = \Cmid$, and $\Wmid = \Cmid$ 

\end{enumerate}

Whenever Wmid with AC(L) and observationally matches $Cmid$
then there is a session Amid such that indeed matches.

\item
$M$ guarantees
\emph{Only Handled by Authorized Party/Operator to a $N$ card $C$} if,
whenever $C$ has a session $(\Cini, \Cmid, \Cfin)$ (or partial) then
there is an OP with session $(\Wini, \Wmid, \Wfin)$ and matching  
taps. Also for partial sessions but matching taps only when complete.

Wmid!!
\end{definition}

Mid tap has been carrie out with authentic card 2nd tap.
Guarantee to A: as long as it's auhentic card guaranteed to be
second tap.


The latter follows if GU OP uses same card as for first, and
okay, and no bla attack. 

and no ghost attacks.

\begin{definition}[OP]
\item Crux
OP carries out $\Wmid$ with authentic $A$.
\end{definition}

\begin{definition}[to OP]
whenever OP has session $(....)$ with $C$ and for them with GU, AC, GU
then card $C$ is authentic and w taps coincide with C taps.
\end{definition}

matches Wtap matches Utap/Atap when successful tap on display
and U guarantted in that state.

if leech tap with C before OP tap with AC, this will be noticed
by AC. leech tap after OP tap with AC not possible due to crypto.
"at the same time" (dual attack) or operator tricks: 2 cards or
no AC tap or ignore error.


Only GU Op performs 2nd tap, and does it after successful
1st tap, i.e. in session $(mid, ) $

no ghost attack, and $OP$ presents authentic card.




==> plain-2/conds-save15.tex <==
\subsection{Authenticity of TAGA Transport}
only one device matches tap
gini = DH session msg agree

\begin{definition}[Guarantees to GU]
We say $N$ guarantees
\emph{`authenticity of initial tap to a GU $G$'} if, whenever $G$
has a session $(S, \Gini, \ldots)$ then there is an authentic card $C$ 
with a session $(\Cini, \ldots)$ such that 
\begin{enumerate}
\item $\nfcl{\Gini}{\Cini}$ and $\msg(\Gini) = \msg(\Cini)$, and
\item $C$ is proximate during the NFC comm. OR: $C$ is the $G$ card. 
\end{enumerate}
\item
We say $N$ guarantees \emph{`authenticity of final tap to a GU $G$'} if,
whenever $G$ has a session $(S, \Gini, \Gfin, \ldots)$ and `authenticity
of initial tap is guaranted to $G$' then there is an authentic card 
$C$ with a session $(\Cini, \Cmid, \Cfin)$ such that 
\begin{enumerate}
\item $\nfcl{\Gini}{\Cini}$, 
\item $\nfcl{\Gfin}{\Cfin}$ and $\msg(\Gfin) = \msg(\Cfin)$, 
\item and $C$ is proximate during the NFC comm. NEED? 
\end{enumerate}
\end{definition}


\begin{definition}[Guarantees to Card]
We say $N$ guarantees
\emph{`integrity of a $N$ card $C$'} if, whenever $C$ has a session
$(\Cini, \Cmid, \Cfin)$ then 
\begin{enumerate}
\item $\msgr(\Cini) = \msgs(\Cmid)$, and
\item $\msgr(\Cmid) = \msgs(\Cfin)$. 
\end{enumerate}
And similarly for partial sessions.
\item
We say $N$ guarantees
\emph{`authenticity of initial tap to a $N$ card $C$'} if, whenever $C$
has a session $(\Cini, \ldots)$ then there is some GU $G$ with
a session $(S, \Gini, \ldots)$ such hat 
\begin{enumerate}
\item $\nfcl{\Cini}{\Gini}$, and $\msg(\Cini) = \msg(\Gini)$, and
\item $C$ is proximate to $G$ during the NFC comm. OR: $C$ is the $G$ card.
\end{enumerate}
\item
We say $N$ guarantees
\emph{`authenticity of middle tap to a $N$ card $C$} if, whenever
$C$ has a session $\Cini, \Cmid, \ldots)$ and $\partner(\Cmid)$ is
an AC $A$ then $A$ has a session $(\Amid, \ldots)$ such that
$\nfcl{\Cmid}{\Amid}$ and $\msg(\Cmid) = \msg(Amid)$. 
\item
We say $N$ guarantees
\emph{`authenticity of final tap to a $N$ card $C$'} if, whenever
$C$ has a session $(\Cini, \Cmid, \Cfin)$ and `authenticity
of initial tap' is guaranteed to $C$ then there is some GU $G$ 
with a session $(S,\Gini,\Gfin, \ldots)$ such that 
\begin{enumerate}
\item $\nfcl{\Cini}{\Gini}$, 
\item $\nfcl{\Cfin}{\Gfin}$ and $\msgs(\Cfin) = \msgr(Gfin)$
\end{enumerate}
\end{definition}

\begin{definition}[Guarantees to AC]
Let $N$ be an NFC system.
\item
We say $N$ guarantees \emph{`proximity of NFC link to an AC $A$'} if,
whenever an AC $A$ has a session $(\Amid, \ldots)$ then $\partner(\Amid)$
is proximate to $A$.
\item
We say $N$ guarantees \emph{`authenticity of mid tap with 
authentic card to an AC $A$'}, if
whenever $A$ has a session $(\Amid, \ldots)$ and $\partner(\Amid)$
is an authentic card $C$ then $C$ has a session 
$(\Cini, \Cmid, \ldots)$ such that 
$\nfcl{\Amid}{\Cmid}$ and $\msg(\Amid) = \msg(\Cmid)$.
\end{definition}

\begin{enumerate}
\item Only a OP can be proximate to a GU.

\item Operators do taps only as part of taga sessions.
\end{enumerate}

matches Wtap matches Utap/Atap when successful tap on display
and U guarantted in that state.

if leech tap with C before OP tap with AC, this will be noticed
by AC. leech tap after OP tap with AC not possible due to crypto.
"at the same time" (dual attack) or operator tricks: 2 cards or
no AC tap or ignore error.


Only GU Op performs 2nd tap, and does it after successful
1st tap, i.e. in session $(mid, ) $

no ghost attack, and $OP$ presents authentic card.


Concluding between Gtaps and Wtaps.
\emph{Origin Authenticity of Proximate NFC Exchange}

\begin{proposition}
\label{prop:nfc}
\item
If a GU has a NFC link $\Gx$ and $\partner(\Gx)$ is proximate then
there is an operator tap $\Wx$ such that
\begin{enumerate}
\item $\card(\Wx) = \partner(\Gx)$, and
\item $\tapl{\Wx}{\Gx}$.
\end{enumerate}
\item
If there is an operator tap $\Wx$ and $\reader(\Wx)$ is a GU $G$
then $G$ has a NFC link $\Gx$ such that
\begin{enumerate}
\item $\card(\Wx) = \partner(\Gx)$, and
\item $\tapl{\Wx}{\Gx}$.
\end{enumerate}
\item
The definitions for an AC $A$ are analogous.
\end{proposition}

\begin{proof}
(2) only proximate exchange and at most one device proximate during
tap.
\end{proof}

\begin{fact}
\label{fact:firstTap}
\begin{enumerate}
\item If $\tapl{W}{\Gini}$ and $\Gini$ is first NFC link of a GU session
then operator of tap has a session $(\Wini, ...)$.
i.e. this is first tap ofa taga session.
\item If $\tapl{\Wini}{Gx}$ and $\Wini$ is a first tap of a session
      $(\Wini, \ldots)$ then $Gx$ is the first NFC link of a GU
      session $(Gx, \ldots)$.

\item also for 2: show the same, since 1 C session.
\end{enumerate}
\end{fact}

Taps only as part of TAGA sessions:

\begin{fact}[Taps and operator sessions]
\label{fact:tapsWalk}
\begin{enumerate}
\item If there are operator taps $\Wx$ and $\Wy$ such that
   for some GU $G$ with session $(\Gini, \Gmid, \Gfin)$
   we have $\tapl{\Wx}{\Gini}$ and $\tapl{\Wy}{\Gfin}$ then
   there must be an operator session $(\Wx, \Wmid, \Wy)$ for
    some $\Wmid$.

\item If there is an operator tap $\Wx$ such that $\reader(\Wx) = A$
      for some AC $A$ then there is an operator session
      $(\Wini, \Wx, \ldots)$ for some $\Wini$.
\end{enumerate}
\end{fact}

\begin{fact}[Operator session]
\label{fact:walk}
Given an operator session $(\Wini, \Wmid, \ldots)$ we have:
\begin{enumerate}
\item $\reader(\Wini)$ is a GU $G$,
\item $\reader(\Wmid)$ is a AC $A$,
\item the location of $G$ and $A$ is the same,
\item $\card(\Wini) = \card(\Wmid)$,
\item There are no taps with $C$ to $G$ between $\Wini$ and
      $\Wmid$.
\end{enumerate}
\end{fact}

\begin{theorem}
If a NFC system satisfies ... then it guarantees Authenticity.
\end{theorem}

\begin{proof}[Proof of Authenticity]
\emph{Guarantee for GU:}
Assume $G$ has a session $(S, \Gini, \Gfin, ?)$ at $L$ then
by `authenticity of initial and final tap to $G$' there is an
\emph{authentic} card $C$ with a session $(\Cini, \Cmid, \Cfin)$
such that the NFC ssns and exchanged messages are matching: i.e.\
$\nfcl{\Gini}{\Cini}$ and $\msg(\Gini) = \msg(\Cini)$, and
$\nfcl{\Gfin}{\Cfin}$ and $\msg(\Gfin) = \msg(\Cfin)$;
and $C$ is proximate to $G$ during each link.

By Prop.~\ref{prop:nfc}(1) there are operator taps $\Wini$, $\Wfin$
such that $\card(\Wini) = C$ and $\tapl{\Wini}{\Gini}$, and
$\card(\Wfin) = C$ and $\tapl{\Wfin}{\Gfin}$. Then by
Fact~\ref{fact:tapsWalk}(1) there is an operator with a session 
$(\Wini, \Wmid, \Wfin)$ for some $\Wmid$.

Then by Fact~\ref{fact:walk}
we have $\reader(\Wmid) = \AC(L)$ and $\card(\Wmid) = C$.
Hence, by Prop~\ref{prop:nfc}(2) $A$ has a session $(\Amid, \ldots)$
such that $\partner(\Amid) = C$ and $\tapl{\Wmid}{\Amid}$.
Let $\Cx$ be defined by $\nfcl{\Amid}{\Cx}$.
$\Cx$ takes place after $\Gini$ (and hence $\Cini$) and before $\Gfin$ 
(and hence $\Cfin$). Since $C$ cannot finish its session without a
second NFC ssn wih $G$ (PROP), and by Fact~\ref{fact:walk}(5)
there can't be any NFC links with $G$ between $\Gini$ and $\Gfin$ 
$\Cx$ must be in the same card session as $\Cini$ and $\Cfin$.
Hence, we conclude that $\Cx = \Cmid$.
Then by `authenticity of mid tap with authentic card to AC' 
we also have $\msg(Ax) = \msg(\Cmid)$. 
Finally, by Integrity of $C$ it is straightforward to check that
the messages of the $A$ session match those of the $G$ session.

\emph{Guarantee for AC:}
Assume $A$ at $L$ has a session $(\Amid, \ldots)$. Then by
`Proximity of NFC Peer' $\partner(\Amid)$, say $C$, is proximate.
Then by Prop.~\ref{prop:nfc}(1) there is an operator tap $\Wx$
such that $\tapl{\Wx}{\Amid}$ and $\card(\Wx) = C$.
Then by Fact~\ref{fact:tapsWalk}(2) there is an operator with
session $(\Wini, \Wx, ...)$ for some $\Wini$. By Fact~\ref{fact:walk}
$\reader(\Wini)$ is a GU $G$ at $L$, and $\card(\Wini) = C$.

By Prop.~\ref{prop:nfc}(2) $G$ has a NFC link $\Gx$ such that
$\partner(\Gx) = C$, and $\tapl{\Wini}{\Gx}$.
Then by Fact~\ref{fact:firstTap}(2) $G$ has a session $(\Gx, \ldots)$.
Then by `authenticity of first tap to $G$' there is an authentic
card $C'$ with a session
$(\Cx, \ldots)$ such that $\nfcl{\Gx}{\Cx}$ and $\msg(\Gx) = \msg(\Cx)$.
Since $\partner(\Gx) = C$ we obtain $C' = C$, and hence, 
$C$ must be authentic.

Since $C$ is authentic by `authenticity of mid tap to AC' $C$ has
a session $(\Cini, \Cmid, \ldots)$ such that $\nfcl{\Amid}{\Cmid}$
and the messages match. Since the session $(\Cx, \ldots)$ can only be closed
by another tap with $G$ and by Fact~\ref{fact:walk}(5) there can't be
any NFC links with $G$ between $\Cini$ and $\Cmid$, we must have 
$\Cini = \Cx$.  By Integrity of $C$ this also means the
messages of $\Amid$ and $\Gx$ are matching.
\end{proof}



==> plain-2/conds-save17.tex <==
\subsection{Authenticity of TAGA Transport}
only one device matches tap
gini = DH session msg agree

$<$ earlier than

From Assumption:
Then obtain: if $\nfcl{s1}{s2}$ then $\msg(s_1) = \msg(s_2)$

We say a reader or a tag have a \emph{NFC session (NFC ssn)}
when they are mapped and exchange data over the link. TODO
At most linked to one device. events.
If a reader $R$ has a ssn $\Rx$ and a tag $C$ has a ssn $\Cy$
and $R$ and $C$ communicate with each other during these sessions
then we write this by $\nfcl{\Rx}{\Cy}$.
TODO partner(R) is a function.


\begin{definition}[Guarantees to GU]
Let $N$ be a NFC system.
\item
We say $N$ guarantees \emph{`authenticity of initial tap to a GU $G$'} if,
whenever $G$ has a session $(S, \Gini, \ldots)$ 
then there is an \emph{authentic} card $C$ with a session 
$(\Cini, \ldots)$ such that 
\begin{enumerate}
\item $\nfcl{\Gini}{\Cini}$ and $\msg(\Gini) = \msg(\Cini)$, and
\item $C$ is proximate to $G$ during $\Cini$.
\end{enumerate}
\item
We say $N$ guarantees \emph{`authenticity of final tap to 
a GU $G$'} if, whenever $G$ has a session $(S, \Gini, \Gfin, \ldots)$ 
then there is an authentic card 
$C$ with a session $(\Cini, \Cmid, \Cfin)$ such that 
\begin{enumerate}
\item $\nfcl{\Gini}{\Cini}$ and $\msg(\Gini) = \msg(\Cini)$,
\item $\nfcl{\Gfin}{\Cfin}$ and $\msg(\Gfin) = \msg(\Cfin)$, and
\item $C$ is proximate to $G$ during $\Cini$ and $\Cfin$.   
\end{enumerate}
\end{definition}

\begin{definition}[Guarantees to Card]
Let $N$ be a NFC system.
\item
We say $N$ guarantees
\emph{`integrity of a $N$ card $C$'} if, whenever $C$ has a session
$(\Cini, \Cmid, \Cfin)$ then 
\begin{enumerate}
\item $\msgr(\Cini) = \msgs(\Cmid)$, and
\item $\msgr(\Cmid) = \msgs(\Cfin)$. 
\end{enumerate}
And similarly for partial sessions.
\item
We say $N$ guarantees
\emph{`authenticity of initial tap to a card $C$'} if, whenever $C$
has a session $(\Cini, \ldots)$ then there is some GU $G$ with
a session $(S, \Gini, \ldots)$ such hat 
\begin{enumerate}
\item $\nfcl{\Gini}{\Cini}$, and $\msg(\Gini) = \msg(\Cini)$, and
\item $C$ is proximate to $G$ during $\Cini$.
\end{enumerate}
\item
We say $N$ guarantees
\emph{`authenticity of mid tap with AC to a card $C$} if, whenever
$C$ has a session $(\Cini, \Cmid, \ldots)$ and $\partner(\Cmid)$ is
an AC $A$ then $A$ has a session $(\Amid, \ldots)$ such that
$\nfcl{\Amid}{\Cmid}$ and $\msg(\Amid) = \msg(\Cmid)$. 
\removed{
\item
We say $N$ guarantees
\emph{`authenticity of final tap to a $N$ card $C$'} if, whenever
$C$ has a session $(\Cini, \Cmid, \Cfin)$ and `authenticity
of initial tap' is guaranteed to $C$ then there is some GU $G$ 
with a session $(S,\Gini,\Gfin, \ldots)$ such that 
\begin{enumerate}
\item $\nfcl{\Cini}{\Gini}$, 
\item $\nfcl{\Cfin}{\Gfin}$ and $\msgs(\Cfin) = \msgr(Gfin)$
\end{enumerate}
}
\end{definition}

\begin{definition}[Guarantees to AC]
Let $N$ be an NFC system.
\item
We say $N$ guarantees \emph{`proximity of NFC peer to an AC $A$'} if,
whenever an AC $A$ has a session $(\Amid, \ldots)$ 
then $\partner(\Amid)$ is proximate to $A$ during $\Amid$.
\item
We say $N$ guarantees \emph{`authenticity of mid tap with an authentic 
card to an AC $A$'}, if
whenever $A$ has a session $(\Amid, \ldots)$ and $\partner(\Amid)$
is an authentic card $C$ then $C$ has a session 
$(\Cini, \Cmid, \ldots)$ such that 
$\nfcl{\Amid}{\Cmid}$ and $\msg(\Amid) = \msg(\Cmid)$.
\end{definition}

\begin{proposition}
\label{prop:nfc}
\item
\begin{enumerate}
\item
If a GU or AC reader $R$ has a NFC ssn $\Rx$ and $\partner(\Rx)$ is 
proximate during $\Rx$ then there is an operator tap $\Wx$ such that
\begin{enumerate}
\item $\card(\Wx) = \partner(\Rx)$, and
\item $\tapl{\Wx}{\Rx}$.
\end{enumerate}
\item
If there is an operator tap $\Wx$ and $\reader(\Wx)$ is a GU or
AC reader $R$ then $R$ has a NFC ssn $\Rx$ such that
\begin{enumerate}
\item $\card(\Wx) = \partner(\Rx)$, and
\item $\tapl{\Wx}{\Rx}$.
\item If $R$ is a GU reader then $C$ is authentic.
\end{enumerate}
\end{enumerate}
\end{proposition}

\begin{proof}
(1)~This follows from `secure proximate zone'.

(2)~Since the operator visually verifies that the reader has 
successfully completed an NFC exchange (e.g.~green light) $\Rx$ exists.
By `secure proximate zone' the exchange must have indeed been carried
out with the operator's card. If the reader is a GU the GU will
check authenticity of the card during the exchange, and the
NFC exchange will fail if it is not (e.g.~red light). 
\end{proof}

\paragraph*{Operator}

  i.e.\ presses abort button after display information.

\begin{enumerate}
\item When an operator performs a tap $\Wx$ with the reader of a
GU $G$ and $G$'s reader displays that a new TAGA session is initialized then 
either the operator is on a TAGA walk/has a TAGA session $(\Wx, \ldots)$
or he will abort $G$'s session before carrying out any further taps with $G$.

\item When an operator is on a TAGA walk/session $(\Wini, \ldots)$ 
and carries out the mid tap with the reader of an AC $A$ then either
the tap is successful (e.g.\ green light) or the operator aborts 
the session of $\reader(\Wini)$ before carrying out any further
taps with that GU.

\item An operator taps an AC only as part of the mid tap of a TAGA session.
\end{enumerate} 

\paragraph*{Taps and ssns }

\begin{fact}[Taps and operator sessions]
\label{fact:tapsWalk}
\item
\begin{enumerate}
\item If there are operator taps $\Wx$ and $\Wy$ and a GU
      session $(S, \Gini, \Gfin, \ldots)$ such that
      $\tapl{\Wx}{\Gini}$ and $\tapl{\Wy}{\Gfin}$ then
      there must be an operator session $(\Wx, \Wmid, \Wy)$ for
      some $\Wmid$.

\item If there is an operator tap $\Wac$ and an AC session 
      $(\Amid, \ldots)$ such that $\tapl{\Wac}{\Amid}$ then 
      there must be an operator session 
      $(\Wini, \Wac, \ldots)$ for some $\Wini$.
\end{enumerate}
\end{fact}

\begin{proof}
(1) By (1) the operator will immediately abort the GU session if $\Wx$
wasn't the first tap of a TAGA session $(\Wx, \ldots)$. Since $G$
receives the last NFC ssn the latter must be true. 
By WALK the operator will carry on to the AC. By (2) the tap is
either successful or the operator will immediately abort 
$G$'s session. Since $G$ receives the last NFC ssn the former must
be true. But then $\Wmid$ exists as required. 

(2) This follows by (3).
\end{proof}

\begin{proof}
(1) $\Gini$ initiates an OP session $(\Wx, \ldots)$.
Since $\Gfin$ the operator has not aborted the session. Then
the OP has completed a walk $(\Wini, \Wmid, \Wfin)$. 
with one $C$ at most one comm, must have happened with $\Wmid$.
only one tap.
\end{proof}


\begin{theorem}
Let $N$ be an NFC system, and $M$ a set of process measures.
If $N$ guarantees the guarantees to GU, AC, and card,
and $M$ includes `abort measures' and `secure proximate zone'
then $N$ under $M$ guarantees Channel Authenticity.
\end{theorem}

\begin{proof}[Proof of Authenticity]
\emph{Guarantee for GU:}
Assume $G$ has a session $(S, \Gini, \Gfin, \ldots)$. Then
by `authenticity of final tap to $G$' there is an
\emph{authentic} card $C$ with a session $(\Cini, \Cmid, \Cfin)$
such that the NFC ssns and exchanged messages are matching, i.e.: 
$\nfcl{\Gini}{\Cini}$, $\nfcl{\Gfin}{\Cfin}$, $\msg(\Gini) = \msg(\Cini)$, 
and $\msg(\Gfin) = \msg(\Cfin)$. Moreover, $C$ is proximate to $G$ 
during $\Cini$ and $\Cfin$.

By Prop.~\ref{prop:nfc}(1) there are successful operator taps $\Wini$, $\Wfin$
such that $\card(\Wini) = C$ and $\tapl{\Wini}{\Gini}$, and
$\card(\Wfin) = C$ and $\tapl{\Wfin}{\Gfin}$ respectively. Then by
Fact~\ref{fact:tapsWalk}(1) there is an operator with a session 
$(\Wini, \Wmid, \Wfin)$ for some $\Wmid$.

Further, by definition of OP session we obtain $\reader(\Wmid) = A$ for
some AC $A$ and $\card(\Wmid) = C$. Hence, by Prop~\ref{prop:nfc}(2) 
$A$ has a successful NFC ssn $\Aac$ such that $\partner(\Aac) = C$ and 
$\tapl{\Wmid}{\Aac}$.
Let $\Cac$ be defined by $\nfcl{\Aac}{\Cac}$. 
$\Cac$ takes place after $\Gini$ (and hence $\Cini$) and before $\Gfin$ 
(and hence $\Cfin$). Hence, we conclude that $\Cac = \Cmid$.
Then by `authenticity of mid tap with AC to $C$' $A$ must have
a session $(\Amid, \ldots)$ and  $\msg(\Amid) = \msg(\Cmid)$. 
Finally, by `integrity of $C$' it is straightforward to check that
the messages of the $A$ session match those of the $G$ session.

\emph{Guarantee for AC:}
Assume $A$ has a session $(\Amid, \ldots)$. Then by
`proximity of NFC peer to $A$' $\partner(\Amid)$, say $C$, is proximate.
Then by Prop.~\ref{prop:nfc}(1) there is a successful operator tap $\Wac$
such that $\tapl{\Wac}{\Amid}$ and $\card(\Wac) = C$.
Then by Fact~\ref{fact:tapsWalk}(2) there is an operator with
session $(\Winiac, \Wac, \ldots)$ for some $\Winiac$. By definition of
OP session
$\reader(\Winiac)$ is a GU $\Gac$, and $\card(\Winiac) = C$.

By Prop.~\ref{prop:nfc}(2) $\Gac$ has a successful NFC ssn $\Giniac$ such that
$\partner(\Giniac) = C$, $\tapl{\Winiac}{\Giniac}$, and $C$ is authentic.
Let $\Ciniac$ be defined by $\nfcl{\Giniac}{\Ciniac}$.

Since $C$ is authentic by `authenticity of mid tap with authentic
card to $A$' $C$ has a session $(\Cini, \Cmid, \ldots)$ such 
that $\nfcl{\Amid}{\Cmid}$ and $\msg(\Amid) = \msg(\Cmid)$.
By `authenticity of first tap to $C$' there is some GU $G$ with a session 
$(S, \Gini, \ldots)$ such that $\nfcl{\Gini}{\Cini}$,
$\msg(\Gini) = \msg(\Cini)$, and $C$ is proximate to $G$ during
$\Cini$. By `integrity of $C$' we also obtain that the messages of $\Amid$ and 
$\Gini$ are matching. 

Moreover, by Prop.~\ref{prop:nfc}(1) there is a successful operator
tap $\Wini$ such that $\card(\Wini) = C$ and $\tapl{\Wini}{\Gini}$.
Hence, it only remains to show that $\Wini = \Winiac$. 
To the contrary assume this not to be the case.
Then by definition of OP session, clause~(5) $\Wini < \Winiac$, and hence 
$\Cini < \Ciniac$. But this leads to a contradication:
since $\tapl{\Wac}{\Cmid}$ and $\Cini$ immediately precedes
$\Cmid$ on $C$, we must have $\Ciniac < \Cini$.
\end{proof}



==> plain-2/conds-text.tex <==

\begin{enumerate}
\item Only a OP can be proximate to a GU.

\item Operators do taps only as part of taga sessions.
\end{enumerate}

matches Wtap matches Utap/Atap when successful tap on display
and U guarantted in that state.

if leech tap with C before OP tap with AC, this will be noticed
by AC. leech tap after OP tap with AC not possible due to crypto.
"at the same time" (dual attack) or operator tricks: 2 cards or
no AC tap or ignore error.


Only GU Op performs 2nd tap, and does it after successful
1st tap, i.e. in session $(mid, ) $

no ghost attack, and $OP$ presents authentic card.


Concluding between Gtaps and Wtaps.
\emph{Origin Authenticity of Proximate NFC Exchange}



==> plain-2/conds12.tex <==
\subsection{Authenticity of TAGA Transport}

$M$ must guarantee `secure proximate zone'

Due to `secure proximate zone' and distance bounding we
can infer operator taps from NFC ssns of the GU and AC reader, 
and vice versa.

\begin{proposition}
\label{prop:nfc}
\item
\begin{enumerate}
\item
If a GU or AC reader $R$ has a NFC ssn $\Rx$ and $\partner(\Rx)$ is
proximate during $\Rx$ then there is an operator tap $\Wx$ such that
\begin{enumerate}
\item $\card(\Wx) = \partner(\Rx)$, and
\item $\tapl{\Wx}{\Rx}$.
\end{enumerate}
\item
If there is an operator tap $\Wx$ and $\reader(\Wx)$ is a GU or
AC reader $R$ then $R$ has a NFC ssn $\Rx$ such that
\begin{enumerate}
\item $\card(\Wx) = \partner(\Rx)$, and
\item $\tapl{\Wx}{\Rx}$.
\item If $R$ is a GU reader then $C$ is authentic.
\end{enumerate}
\end{enumerate}
\end{proposition}

\begin{proof}
(1)~This follows from `secure proximate zone'.

(2)~Since the operator visually verifies that the reader has
successfully completed an NFC exchange (e.g.~green light) $\Rx$ exists.
By distance bounding and 
`secure proximate zone' the exchange must have indeed been carried
out with the operator's card. If the reader is a GU the GU will
check authenticity of the card during the exchange, and the
NFC exchange will fail if it is not (e.g.~red light).
\end{proof}

The following are guarantees that the NFC system provides to
the GU, card, and AC.


%Then obtain: if $\nfcl{s1}{s2}$ then $\msg(s_1) = \msg(s_2)$
Let $E$ be a set of NFC sessions (NFC ssns). During NFC
there is only one active field.
A reader has selected one tag it assumes to talk to,
parnter(n). A tag assumes to talk to one active reader.
partner(n). When

If a reader $R$ has a ssn $\Rx$ and a tag $C$ has a ssn $\Cy$
and $R$ and $C$ communicate with each other during these sessions
then we write this by $\nfcl{\Rx}{\Cy}$.

A (TAGA) session of a card $C$ is a tuple $(\Cini, \Cmid, \Cfin)$
such that $\msgr(\Cini) = \msgs(\Cmid)$, and
$\msgr(\Cmid) = \msgs(\Cfin)$. 

\begin{definition}[Guarantees to GU]
Let $N$ be a NFC system.
\item
We say $N$ guarantees \emph{`authenticity of initial tap to a GU $G$'} if,
whenever $G$ has a session $(S, \Gini, \ldots)$ 
then there is an \emph{authentic} card $C$ with a session 
$(\Cini, \ldots)$ such that 
\begin{enumerate}
\item $\nfcl{\Gini}{\Cini}$ and $\msg(\Gini) = \msg(\Cini)$, and
\item $C$ is proximate to $G$ during $\Cini$.
\end{enumerate}
\item
We say $N$ guarantees \emph{`authenticity of final tap to 
a GU $G$'} if, whenever $G$ has a session $(S, \Gini, \Gfin, \ldots)$ 
then there is an authentic card 
$C$ with a session $(\Cini, \Cmid, \Cfin)$ such that 
\begin{enumerate}
\item $\nfcl{\Gini}{\Cini}$ and $\msg(\Gini) = \msg(\Cini)$,
\item $\nfcl{\Gfin}{\Cfin}$ and $\msg(\Gfin) = \msg(\Cfin)$, and
\item $C$ is proximate to $G$ during $\Cini$ and $\Cfin$.   
\end{enumerate}
\end{definition}

\begin{definition}[Guarantees to Card]
Let $N$ be a NFC system.
\removed{
\item
We say $N$ guarantees
\emph{`integrity of a $N$ card $C$'} if, whenever $C$ has a session
$(\Cini, \Cmid, \Cfin)$ then 
\begin{enumerate}
\item $\msgr(\Cini) = \msgs(\Cmid)$, and
\item $\msgr(\Cmid) = \msgs(\Cfin)$. 
\end{enumerate}
And similarly for partial sessions.}
\item
We say $N$ guarantees
\emph{`authenticity of initial tap to a card $C$'} if, whenever $C$
has a session $(\Cini, \ldots)$ then there is some GU $G$ with
a session $(S, \Gini, \ldots)$ such hat 
\begin{enumerate}
\item $\nfcl{\Gini}{\Cini}$, and $\msg(\Gini) = \msg(\Cini)$, and
\item $C$ is proximate to $G$ during $\Cini$.
\end{enumerate}
\item
We say $N$ guarantees
\emph{`authenticity of mid tap with AC to a card $C$} if, whenever
$C$ has a session $(\Cini, \Cmid, \ldots)$ and $\partner(\Cmid)$ is
an AC $A$ then $A$ has a session $(\Amid, \ldots)$ such that
$\nfcl{\Amid}{\Cmid}$ and $\msg(\Amid) = \msg(\Cmid)$. 
\removed{
\item
We say $N$ guarantees
\emph{`authenticity of final tap to a $N$ card $C$'} if, whenever
$C$ has a session $(\Cini, \Cmid, \Cfin)$ and `authenticity
of initial tap' is guaranteed to $C$ then there is some GU $G$ 
with a session $(S,\Gini,\Gfin, \ldots)$ such that 
\begin{enumerate}
\item $\nfcl{\Cini}{\Gini}$, 
\item $\nfcl{\Cfin}{\Gfin}$ and $\msgs(\Cfin) = \msgr(Gfin)$
\end{enumerate}
}
\end{definition}

\begin{definition}[Guarantees to AC]
Let $N$ be an NFC system.
\item
We say $N$ guarantees \emph{`proximity of NFC peer to an AC $A$'} if,
whenever an AC $A$ has a session $(\Amid, \ldots)$ 
then $\partner(\Amid)$ is proximate to $A$ during $\Amid$.
\item
We say $N$ guarantees \emph{`authenticity of mid tap with an authentic 
card to an AC $A$'}, if
whenever $A$ has a session $(\Amid, \ldots)$ and $\partner(\Amid)$
is an authentic card $C$ then $C$ has a session 
$(\Cini, \Cmid, \ldots)$ such that 
$\nfcl{\Amid}{\Cmid}$ and $\msg(\Amid) = \msg(\Cmid)$.
\end{definition}

\begin{proposition}
\label{prop:nfc}
\item
\begin{enumerate}
\item
If a GU or AC reader $R$ has a NFC ssn $\Rx$ and $\partner(\Rx)$ is 
proximate during $\Rx$ then there is an operator tap $\Wx$ such that
\begin{enumerate}
\item $\card(\Wx) = \partner(\Rx)$, and
\item $\tapl{\Wx}{\Rx}$.
\end{enumerate}
\item
If there is an operator tap $\Wx$ and $\reader(\Wx)$ is a GU or
AC reader $R$ then $R$ has a NFC ssn $\Rx$ such that
\begin{enumerate}
\item $\card(\Wx) = \partner(\Rx)$, and
\item $\tapl{\Wx}{\Rx}$.
\item If $R$ is a GU reader then $C$ is authentic.
\end{enumerate}
\end{enumerate}
\end{proposition}

\begin{proof}
(1)~This follows from `secure proximate zone'.

(2)~Since the operator visually verifies that the reader has 
successfully completed an NFC exchange (e.g.~green light) $\Rx$ exists.
By `secure proximate zone' the exchange must have indeed been carried
out with the operator's card. If the reader is a GU the GU will
check authenticity of the card during the exchange, and the
NFC exchange will fail if it is not (e.g.~red light). 
\end{proof}

\paragraph*{Operator}

  i.e.\ presses abort button after display information.

\begin{enumerate}
\item When an operator performs a tap $\Wx$ with the reader of a
GU $G$ and $G$'s reader displays that a new TAGA session is initialized then 
either the operator is on a TAGA walk/has a TAGA session $(\Wx, \ldots)$
or he will abort $G$'s session before carrying out any further taps with $G$.

\item When an operator is on a TAGA walk/session $(\Wini, \ldots)$ 
and carries out the mid tap with the reader of an AC $A$ then either
the tap is successful (e.g.\ green light) or the operator aborts 
the session of $\reader(\Wini)$ before carrying out any further
taps with that GU.

\item An operator taps an AC only as part of the mid tap of a TAGA session.
\end{enumerate} 

\paragraph*{Taps and ssns }

\begin{fact}[Taps and operator sessions]
\label{fact:tapsWalk}
\item
\begin{enumerate}
\item If there are operator taps $\Wx$ and $\Wy$ and a GU
      session $(S, \Gini, \Gfin, \ldots)$ such that
      $\tapl{\Wx}{\Gini}$ and $\tapl{\Wy}{\Gfin}$ then
      there must be an operator session $(\Wx, \Wmid, \Wy)$ for
      some $\Wmid$.

\item If there is an operator tap $\Wac$ and an AC session 
      $(\Amid, \ldots)$ such that $\tapl{\Wac}{\Amid}$ then 
      there must be an operator session 
      $(\Wini, \Wac, \ldots)$ for some $\Wini$.
\end{enumerate}
\end{fact}

\begin{proof}
(1) By (1) the operator will immediately abort the GU session if $\Wx$
wasn't the first tap of a TAGA session $(\Wx, \ldots)$. Since $G$
receives the last NFC ssn the latter must be true. 
By WALK the operator will carry on to the AC. By (2) the tap is
either successful or the operator will immediately abort 
$G$'s session. Since $G$ receives the last NFC ssn the former must
be true. But then $\Wmid$ exists as required. 

(2) This follows by (3).
\end{proof}

\begin{proof}
(1) $\Gini$ initiates an OP session $(\Wx, \ldots)$.
Since $\Gfin$ the operator has not aborted the session. Then
the OP has completed a walk $(\Wini, \Wmid, \Wfin)$. 
with one $C$ at most one comm, must have happened with $\Wmid$.
only one tap.
\end{proof}


\begin{theorem}
Let $N$ be an NFC system, and $M$ a set of process measures.
If $N$ guarantees the guarantees to GU, AC, and card,
and $M$ includes `abort measures' and `secure proximate zone'
then $N$ under $M$ guarantees Channel Authenticity.
\end{theorem}

\begin{proof}[Proof of Authenticity]
\emph{Guarantee for GU:}
Assume $G$ has a session $(S, \Gini, \Gfin, \ldots)$. Then
by `authenticity of final tap to $G$' there is an
\emph{authentic} card $C$ with a session $(\Cini, \Cmid, \Cfin)$
such that the NFC ssns and exchanged messages are matching, i.e.: 
$\nfcl{\Gini}{\Cini}$, $\nfcl{\Gfin}{\Cfin}$, $\msg(\Gini) = \msg(\Cini)$, 
and $\msg(\Gfin) = \msg(\Cfin)$. Moreover, $C$ is proximate to $G$ 
during $\Cini$ and $\Cfin$.

By Prop.~\ref{prop:nfc}(1) there are successful operator taps $\Wini$, $\Wfin$
such that $\card(\Wini) = C$ and $\tapl{\Wini}{\Gini}$, and
$\card(\Wfin) = C$ and $\tapl{\Wfin}{\Gfin}$ respectively. Then by
Fact~\ref{fact:tapsWalk}(1) there is an operator with a session 
$(\Wini, \Wmid, \Wfin)$ for some $\Wmid$.

Further, by definition of OP session we obtain $\reader(\Wmid) = A$ for
some AC $A$ and $\card(\Wmid) = C$. Hence, by Prop~\ref{prop:nfc}(2) 
$A$ has a successful NFC ssn $\Aac$ such that $\partner(\Aac) = C$ and 
$\tapl{\Wmid}{\Aac}$.
Let $\Cac$ be defined by $\nfcl{\Aac}{\Cac}$. 
$\Cac$ takes place after $\Gini$ (and hence $\Cini$) and before $\Gfin$ 
(and hence $\Cfin$). Hence, we conclude that $\Cac = \Cmid$.
Then by `authenticity of mid tap with AC to $C$' $A$ must have
a session $(\Amid, \ldots)$ and  $\msg(\Amid) = \msg(\Cmid)$. 
Finally, by definition of session of a card it is straightforward to check that
the messages of the $A$ session match those of the $G$ session.

\emph{Guarantee for AC:}
Assume $A$ has a session $(\Amid, \ldots)$. Then by
`proximity of NFC peer to $A$' $\partner(\Amid)$, say $C$, is proximate.
Then by Prop.~\ref{prop:nfc}(1) there is a successful operator tap $\Wac$
such that $\tapl{\Wac}{\Amid}$ and $\card(\Wac) = C$.
Then by Fact~\ref{fact:tapsWalk}(2) there is an operator with
session $(\Winiac, \Wac, \ldots)$ for some $\Winiac$. By definition of
OP session
$\reader(\Winiac)$ is a GU $\Gac$, and $\card(\Winiac) = C$.

By Prop.~\ref{prop:nfc}(2) $\Gac$ has a successful NFC ssn $\Giniac$ such that
$\partner(\Giniac) = C$, $\tapl{\Winiac}{\Giniac}$, and $C$ is authentic.
Let $\Ciniac$ be defined by $\nfcl{\Giniac}{\Ciniac}$.

Since $C$ is authentic by `authenticity of mid tap with authentic
card to $A$' $C$ has a session $(\Cini, \Cmid, \ldots)$ such 
that $\nfcl{\Amid}{\Cmid}$ and $\msg(\Amid) = \msg(\Cmid)$.
By `authenticity of first tap to $C$' there is some GU $G$ with a session 
$(S, \Gini, \ldots)$ such that $\nfcl{\Gini}{\Cini}$,
$\msg(\Gini) = \msg(\Cini)$, and $C$ is proximate to $G$ during
$\Cini$. By definition of session of a card we also obtain that 
the messages of $\Amid$ and $\Gini$ are matching. 

Moreover, by Prop.~\ref{prop:nfc}(1) there is a successful operator
tap $\Wini$ such that $\card(\Wini) = C$ and $\tapl{\Wini}{\Gini}$.
Hence, it only remains to show that $\Wini = \Winiac$. 
To the contrary assume this not to be the case.
Then by definition of OP session, clause~(5) $\Wini < \Winiac$, and hence 
$\Cini < \Ciniac$. But this leads to a contradication:
since $\tapl{\Wac}{\Cmid}$ and $\Cini$ immediately precedes
$\Cmid$ on $C$, we must have $\Ciniac < \Cini$.
\end{proof}



==> plain-2/db.tex <==

A holder of a cryptographic key proves
to a verifier that it is proximate by answering cryptographic
challenges within a 
Typically this works by the reader (acting
as the verifier) measuring the round-trip time of cryptographic 
challenge/response pairs.

measuring the
round-trip 

protocols. 
 between a verfifier and prover: the holder of a
cryptographic key proves to the verifier that it is proximate
by answering a cryptographic challenge within response time.
If the response time is .. then the verifier concludes must
be proximate.

the card must prove to the reader that it is indeed proximate.

Distance bounding protcols work by measuring the response time
of a cryptographic challenge.

Distance bounding can establish that a device is proximate to
the reader (within ca. 15cm) .. must be bound to the
key though. the holder of a cryptographic key is proximate to
the reader.

Many cards these days implement
Distance bounding protocols, which guarantee an upper bound
on the distance of the card (prover). Typically they work by
measuring the round-trip time of cryptographic challenge/response
pairs. can then be bound to secure channel. (Otherwise danger of
...)



==> plain-2/design.tex <==
\subsection{Designs}

NFC: 

\begin{table}
\begin{tabular}
       &  none  &  bound to $\mcH$ &  bound to $G$ \\
\hline \hline
Robust    &  
\parbox{Secure DB} & 
\end{tabular}
\end{table}

Distribution Model for cards:
Since authenticity is threat it is no option to simply use
a pool of cards. Since it's either too aufwendig to stoare
and distribute securely or too easy to swap a card. 
a.. Hence, it's ownership either with the GU or with the
GU operators, who can use it for any GU.

\begin{design}[personal]

Moreover, the card will then be prone to the usual
relay attacks possible, and we assume distance bounding.
\end{design}



\subsection{NFC Assumptions}

\begin{enumerate}
\item eavesdropping from far (outside ...)
\item while active manip.,
   no mitm attacks, i.e. cannot change on transit while read it
   ourselves. important that never sends the same DH key when repeated
\item leech attacks (fake reader)from ...
\item ghost attacks to reader (fake card)
\end{enumerate}


---
is difficult to manipulate ... 
different, secure zone
Assume: integrity of card.

NFC Device infiltration: for NFC channel attacks
\begin{enumerate}
\item swap the TAGA card while the op is .. during a break etc.
      or when stored ...
\item plant smaller NFC devices onto the OP or equipment of the secure
      zone
\item plant a larger device such as acamouflaged antenna
      outside (and possibly even inside) the secure zone
\item compromise general-purpose NFC-capable devices  such as phones 
\end{enumerate}

---

Eavesdropping from far (tool)/phone?

Data aleration

Counterfeit card attack

Ghost attacks from far (impersonate to reader)
       from zone (?)

Leech/Mole attacks (impersonate to card) from far not possible 
  with compromised device 

Leech/Mole attack with multiple sessions

Piggy-back attack, leech or ghost
active/earlier
ensure that this card/or avoid by being early with active parasite
device

Double card attack with GU OP 
(not NFC dependent)

Proximate Piggy-back attack with GU OP
leech/cactive leech
Piggy-front/head-gating

Authentic NFC card can't detect when sth is wrong while
the reader has successfully communicated.

not clear
---

\begin{assumption}
for impersonation only once./piggy back by mobile phone?/general-purpose
device?
a general-purpose device (hackable from a distance) 
can act as a dual-function mole.  

piggy-front 
\end{assumption}

while the GU OP is a trust achnor this arguably ..
key secrecy.


==> plain-2/later.tex <==
A local NFC attack is one that requires physical device
at .. p

\begin{assumption}
\item requires nfc attack./proximity
 A ghost attack cannot be carried out by a standard device.
\end{assumption}

\begin{theorem}
The NFC systems N-GU and $N-personal$  under $M$ guarantee
Authenticity under $M$ up to NFC attack.

The NFC systems $N-GU^{DB}$ and $N-OP^{DB}$ under $M$ guarantee Authenticity.
(under assumptions)
\end{theorem}

If we lift one then a relay or ghost attack is necessary.



==> plain-2/plain-save.tex <==
\section{Plain TAGA}

The idea behind plain TAGA is as follows: if the NFC system is chosen 
such that the message exchange during TAGA pairing is guaranteed
to be authentic then the session key can securely be established by
an unauthenticated KE protocol such as the basic DH exchange. The
integration of TAGA pairing into the physical setup will then 
easily ensure that a GU $\widehat{G}$ is physically connected
to an AC $\widehat{A}$ iff a secure channel is established between
the same $\widehat{G}$ and $\widehat{A}$.



\subsection{Concept and Security}

We say a TAGA process $(P, N, M)$ is \emph{unauthenticated/plain} when
the KE protocol $P$ is unauthenticated. It is well-known that
unauthenticated KE protocols can be secure against 
passive adversaries but never against active adversaries. In the
latter case any unauthenticated KE protocol can be undermined by 
impersonation and man-in-the-middle attacks. Hence, the premise
of plain TAGA is that the NFC system $N$ can be chosen so that
the channel generated by the Operator's TAGA taps and transport
of $U$ is authenticated.


NFC system during message transfer 

in the secure environ

that can only eavesdrop against 

A \emph{plain TAGA pairing process} is defined as a triple 
$\mcP = (P, N, M)$ where $P$ is an unauthenticated KE protocol, 
$N$ is a NFC system, and $M$ is a set of process measures. 
The premise behind plain TAGA is that the NFC system $N$ can be
chosen such that the message transfer during TAGA pairing is authentic.
Then the underlying KE protocol $P$ only needs to be secure
against eavesdropping, which is achieved by unauthenticated KE
protocols such as the basic DH exchange. Hence, as a result 
the two endpoints of TAGA pairing will share a secret session key and 
a corresponding secure channel without the need for any PKI.
Since TAGA pairing is carried out beween a GU $G$
and an AC $A$ exactly when $G$ and $A$ are physically connected 
it is also guaranteed that the secure cyber channels established
by plain TAGA exactly match the physical connections.
 
\paragraph*{Channel Authenticity.}
We say that an NFC system $(R_G, R_A, U)$ guarantees 
\begin{enumerate}
\item Channel (Message) Authenticity if, whenever TAGA pairing is
  carried out between a GU $G$ and an AC $A$ then $G$ and $A$ 
  have \emph{matching conversations} wrt to their corresponding 
  TAGA sessions, or a disturbance is carried out.
\item Channel (Origin) Authenticity if, whenever a TAGA session
  is initiated by a NFC tap then the tap is c. carried out with an
  authentic TAGA unit $U$. boh G, A
\end{enumerate}
We say $N$ guarantees channel authenticity 


We say $\mcP$ is \emph{secure} when $P$ guarantees Secrecy and Key Freshness 
against passive adversaries and $N$ is guarantees Channel Authenticity.

\begin{proposition}
Let $\mcP = (P, N, M)$ be a secure plain TAGA process.
If an instance of $\mcP$ is carried out between a GU $G$ of type $S$
and an AC $A$ then $A$ and $G$ will share a secure channel for service 
$S$. (as communic. by G) 
\end{proposition}

This is immediate from the defintion of `Good Order' and 
the previous proposition.

\begin{theorem}
Let $P$ be a setup process. If $P$ satisfies `Good Order',
and the underlying plain TAGA process is secure then $P$ is safe and secure.
\end{theorem}

This is 

\begin{definition}
When $G$ engages into $S$ then $G$ is safely physically connected
to $\AC(L)$. and a taga process has been carried out with 
$\AC(L)$.

When $A$ engages into $S$ then $A$ is safely physically
connected to $n$ GUs $S$ at $L$, say at positions $p_1$, ...
and a taga process has been carried out with the same GUs. 
\end{definition}


\begin{enumerate}
\item \emph{Channel Authenticity} to a GU $G$ if, whenever
$G$ has sent a message $M_1$, and accepted a message $M_2$ 
as first and second message of the same TAGA session then 
there is TAGA unit $U$ such that $U$ has received $M_1$ 
as first message, and transmitted $M_2$ has third tap of the
TAGA same session.

\item to an AC $A$ if, whenever $A$ has read a message $M_1$ and
written a message $M_2$ as TAGA message then there is a TAGA unit
$U$ such that $U$ has writen $M_1$ and read $M_2$ as mid tap
of a TAGA session. 

\item to $U$ if, whenever $U$ reads $M_1$ accepts as first tap then
it writes it as secodn tap, and when it reads $M_2$ as second tap 
it writes it as third tap. 
\end{enumerate}


and an AC $A$ and a TAGA unit $U$ such that 0 

 
there is a AC $A$ and a authentic TAGA device $U,$ such that


\begin{itemize}
\item $M_1$ has been read by an authentic TAGA device $D$ operated
  by an authentic operator,
been received by  

\end{itemize}

during TAGA 
pairing is authentic then a 
between a GU and an AC is guaranteed
to be authentic then a key can securely be established by an unauthenticated
KE protocol such as the basic DH exchange.
then  

guarantees an authenticated
message exchange between $\widehat(G)$ and $\widehat{A}$ the respective GU and AC then a key can 
securely be established by an unauthenticated KE protocol such as
the basic DH exchange.  
such that 

when during the setup process
of ground service $S$ a GU $\widehat{G}$ is physically connected to the AC 
$\widehat{A}$ then at the same time TAGA pairing is carried out 
between $\widehat{G}$ and $\widehat{A}$. Moreover, 
if the TAGA transport 
guarantees an authenticated message exchange between two TAGA endpoints 
such as $\widehat{G}$ and $\widehat{A}$ then a key can securely be 
established by an unauthenticated KE protocol such as the basic DH exchange.  

establish a key beween the same entities  
take place between the same physical entities. 
the integration of
TAGA pairing ensures that a key is established

physical connection
is set up between a GU $\widehat{G}$ and AC(L) then TAGA pairing will establishe
a key between the same entitites G and A for S. This can securely done
by using an unauthenticated KE protocol because we make sure that
the TAGA transport allows an authenticated message exchange between
G and A.
spans an authenticated channel between 

such as basic DH key exchange 
when we ensure that the 

By ensuring that
the NFC system used  


while the operators
establish the physical connection they 
TAGA pairing will span
a channel 

ensure
that a 




The protocol $P$ is essentialy
the basic DH key exchanwe can base on 
the basic DH key exchange as shown in Fig.~\ref{}. The 
that also communicates the service to $A$ and the ssid to $G$.


When G engages into S then it has physically connected with
S and completed a TAGA process with AC(L).

When A engages into S then it has physically connected to 
n GUs ,,, and to those also taga process.

for S with AC

\begin{theorem}

\end{theorem}

In the prototypical implementation
$P$

We say 
\begin{theorem}
$\mcP$ is secure if $P$ is secure against passive adversaries and
$N$ guarantees  
\end{theorem}


==> plain-2/sols-save.tex <==

\subsection{Designs}

\paragraph*{Distribution Model}
The swap attack shows that authenticity of the card is an
important requirement. Hence, it is advisable that there
is a clear assignment who is responsible for the cards are
when. The card could either be "owned" by the GU, and then
the respective GU operator is responsible for it 
Both of the models have the advantage that authenticity can be
checked by the GU with the initial tap. So both designs 

 The card is ``owned" by the GU. It is stored at the GU (in some
compartment), and the respective GU operator is responsible for 
handling it while operating the GU. 
The card is ``owned" by the operator: Each GU operator is assigned
a card, and is responsible for handling and storing it. It uses it
on the respective GU the operator handles (which can differ from
day to day). This model is particularly suitable when the TAGA
functionality can be integrated into a access card that airport
staff are equipped with in general. 

\paragraph*{Authenticity of Card.}
Both of the models have the advantage that we can add non-central
funcitionality that will provide that authenticity is checked by
the GU with the initial tap. 
Since a \emph{GU-bound card} is specific to the GU, the GU reader
and card can be set up with a shared key $K$. This key $K$ can
then be used for mutual authentication, and also to establish
a fresh key for each TAGA session to secure the communication
over the two NFC links.

If a \emph{personal access card} is used it is likely that the
card contains a public/private key pair that identifies the
card/operator, and the airport maintains a PKI to manage the
corresponding keys and certificates. Then the GU reader can
be set up with corresponding cerificates, that allows it to
check whether it communicates with a regular access card
(and with whom). A fresh key for each session can also be
established based on this.
mutual? 

\paragraph*{Secure against Leech comm./Auth of readercomm. partner}
use the same link
A card only allows one tap between comm. with a GU. And if the
tap with the AC was successful (and indeed NFC link with the card)
then 
While we cannot hinder another device to pretend to be the AC reader.
It cannot pretend to perform teh GU reader.
The AC tap will not be successful, if not a new session has been done. 
If the AC tap was successful the next tap must be with $G$.

\paragraph*{Securing the NFC link between card and the AC.}
NFC security standards (NFC-SEC) define a set of security services
secure channels. This is ..  by NFC-SEC-01 specifies
for use cases when peer NFC devices do not share any common secret.
explicit cryptographic mechanism: ECDH for key agreement and
AES-CTR.. for data encryption and authentication.
``The practical risk of MITM attacks is regarded as low in the
targeted use cases due to the short operating distance and the specific
RF characteristics of NFC'' \cite{}. In bla there is an argument
that passive/active as used a Mitm attack is practically impossible.

\paragraph*{Optional Distance Bounding.}
Distance bounding can establish that a device is proximate to
the reader (within ca. 15cm) .. must be bound to the 
key though.

\paragraph*{Security.}

\begin{table}
\input{plain-2/tab-designs}
\caption{ \label{table}}
\end{table}

\begin{enumerate}
\item GU and AC readers guarantee proximity of $\partner(link)$.
\item $M$ guarantees that any device proximate to a GU or AC 
    reader is a card carried by an OP.
\item OP only bring a card proximate to a GU or AC reader on a regular 
TAGA walk.
\item TAGA walk satisfies certain conditions.
\end{enumerate}    

A local NFC attack is one that requires physical device 
at .. p

\begin{assumption}
\item It is pratically impossible to carry out a man-in-the-middle
attack over NFC. 
\item requires nfc attack./proximity 
 A ghost attack cannot be carried out by a standard device.
\end{assumption}


\begin{theorem}
The NFC systems N-GU and $N-personal$  under $M$ guarantee
Authenticity under $M$ up to NFC attack.

The NFC systems $N-GU^{DB}$ and $N-OP^{DB}$ under $M$ guarantee Authenticity.
(under assumptions) 
\end{theorem}


The proofs are only up to requirements that C, GU and AC reader must
satisfy and informal reasoning why this is possible to implement 
in the above way. only for concrte desigsns.

If we lift one then a relay or ghost attack is necessary.




==> plain-2/sols-save2.tex <==

\subsection{Designs for the NFC System}

\paragraph*{Distribution Model}
The swap attack shows that authenticity of the card is an important 
requirement. Hence, it is advisable that there is not just a pool of 
TAGA cards that are distributed daily to the operators but rather that a
distribution model is in place that allows for accountability.
The following two models offer themselves.

In the `OP-bound model' each GU operator is equipped with their 
personal TAGA card, which she can use on any GU that she is authorized
to operate. This model is particularly suitable when airport staff
are already provided with multi-functional access cards, into which
TAGA can be integrated as one of several applications. The card will
usually contain a public/private key pair that is bound to the
identity of the GU operator and a certificate for the public key
signed by the airport.

In the `GU-bound model' each GU is equipped with its own TAGA card. 
The card can be cryptographically bound to the GU reader so that
the GU can only be operated with its own card, and, conversely, 
the card will only work with the GU that owns it. During operative
times the respective GU operator is responsible for handling it
while during non-operative times it is simply stored within the GU or
within a secure compartment next to the GU reader.

of the security domain she
is 

In the first model each TAGA card is ``owned'' by an operator. 


that each
card is ``owned'' by some. This can be either an operatoran operator or a GU.

someone or something. 

there
is a notion of ownership for each card.

 
card is ``owned'' by either assigned by a GU, or  

 distribution model allows for accountability. 
 
%that are given out to operators
but a distribution model that allows to assign responsibility
for the card. There are two models: \emph{GU-bound} and \emph{OP-bound}.
\emph{A GU-bound card} is ``owned" by the GU. This means in
non-operative times it is stored at the GU (in some
compartment) while during operative times the respective GU operator 
is responsible for handling it. 
An \emph{OP-bound card} is ``owned" by the operator. 
This means each GU operator is provided with a card, and
the card can be used on any GU of the security domain of the operator.
The operator is responsible for handling and storing it. We call
this 
%on the respective GU the operator handles (which can differ from
%day to day).  
This model is particularly suitable when the TAGA
functionality is integrated into an multi-purpose access card that airport
staff are provided with already. 

\paragraph*{Authenticity of the Card}
Both of the models have the advantage that we can add 
functionality that allows the GU to establish the authenticity of the card
with the initial tap. 
Since a \emph{GU-bound card} is specific to the GU, the GU reader
and card can be set up with a shared key $K$. This key $K$ can
then be used for mutual authentication, and also to establish
a fresh key for each TAGA session to secure the communication
over the two NFC links.
%
An \emph{OP-bound card} typically contains a public/private key pair 
that identifies the card and operator. And the airport maintains 
a PKI to manage the corresponding keys and certificates. Then 
the GU reader can be set up with the corresponding root certificates,
and it can authenticate a regular airport card based on its certificate
and private key.  A fresh key for each session can also be established 
based on this.

%certificate check whether whether it communicates with a regular access card
%(and with whom). 
%mutual? 

\paragraph*{Secure against Leech comm./Auth of readercomm. partner}
use the same link
A card only allows one tap between comm. with a GU. And if the
tap with the AC was successful (and indeed NFC link with the card)
then 
While we cannot hinder another device to pretend to be the AC reader.
It cannot pretend to perform teh GU reader.
The AC tap will not be successful, if not a new session has been done. 
If the AC tap was successful the next tap must be with $G$.

\paragraph*{Securing the NFC link between card and the AC.}
NFC security standards (NFC-SEC) define a set of security services
secure channels. This is ..  by NFC-SEC-01 specifies
for use cases when peer NFC devices do not share any common secret.
explicit cryptographic mechanism: ECDH for key agreement and
AES-CTR.. for data encryption and authentication.
``The practical risk of MITM attacks is regarded as low in the
targeted use cases due to the short operating distance and the specific
RF characteristics of NFC'' \cite{}. In bla there is an argument
that passive/active as used a Mitm attack is practically impossible.

\begin{assumption}
\item It is pratically impossible to carry out a man-in-the-middle
attack over NFC. passive/.   
\end{assumption}

Then obtain: if $\nfcl{s1}{s2}$ then $\msg(s_1) = \msg(s_2)$

\paragraph*{Optional Distance Bounding.}
Distance bounding can establish that a device is proximate to
the reader (within ca. 15cm) .. must be bound to the 
key though.

\paragraph*{Security.}

\begin{table}
\input{plain-2/tab-designs}
\caption{ \label{table}}
\end{table}

\begin{enumerate}
\item GU and AC readers guarantee proximity of $\partner(link)$.
\item $M$ guarantees that any device proximate to a GU or AC 
    reader is a card carried by an OP.
\item OP only bring a card proximate to a GU or AC reader on a regular 
TAGA walk.
\item TAGA walk satisfies certain conditions.
\end{enumerate}    

A local NFC attack is one that requires physical device 
at .. p

\begin{assumption}
\item It is pratically impossible to carry out a man-in-the-middle
attack over NFC. 
\item requires nfc attack./proximity 
 A ghost attack cannot be carried out by a standard device.
\end{assumption}


\begin{theorem}
The NFC systems N-GU and $N-personal$  under $M$ guarantee
Authenticity under $M$ up to NFC attack.

The NFC systems $N-GU^{DB}$ and $N-OP^{DB}$ under $M$ guarantee Authenticity.
(under assumptions) 
\end{theorem}


The proofs are only up to requirements that C, GU and AC reader must
satisfy and informal reasoning why this is possible to implement 
in the above way. only for concrte desigsns.

If we lift one then a relay or ghost attack is necessary.




==> plain-2/standards.tex <==

NFC security standards (NFC-SEC) define a set of security services
secure channels. This is ..  by 

NFC-SEC-01 specifies
for use cases when peer NFC devices do not share any common secret.
explicit cryptographic mechanism: 
``The practical risk of MITM attacks is regarded as low in the
targeted use cases due to the short operating distance and the specific
RF characteristics of NFC'' \cite{}. In bla there is an argument
that passive/active as used a Mitm attack is practically impossible.



==> resil/concept.tex <==

\section{Concept of Local Resilience}

In TAGA the setting is \emph{local} in that whenever two
parties 

in that the long term keys anchored in the PKI is to authenticate
parties that are at the same location. 


Two parties that wish to mutually authenticate themselves based
on the lt crdedentials PKI are not remote but always proximate:
they are located at the same parking slot.
We say 

while in such a setting local parties must mutually trust each other,
we also require that conv should not have to trust non-local parties.
we require that they are not affected by security incidences 
in the realm of other airlines or airports. Hence, they should
also have  

This motivates a notion of resilience one would wish to have,
and a means to obtain it.
The notion of resilience is that whenever an AC and  GUs
are involved in the turnaround then they must trust the local
parties each other
but security of the turnaround should not affected by 
security breaches of non-local parties (like in ..).

Since the parties are local we can achieve this by /harden
against LTKCs by local process measures.
This can involve visual monitoring by local staff
(such as GU operators and crew), detection measures built into
the physical entities, local staff reacting to security alerts,
and local channels established by local equipment and staff (such as
the TAGA transport).



TAGA is a \emph{local service} 

In a setting such as TAGA the 

\begin{definition}
Let $T$ be an authenticated TAGA process.
\item
We say $T$ guarantees \emph{$x$ resilience}, where
\emph{$x = \{$domain-reliant, GU-domain-reliant, full$\}$},
if, whenever a ground service that includes $T$ takes place
between AC $A$ and GU $G$ (G1, Gn) then
$T$ guarantees Secure TAGA II to $A$ and $G$ even when, for
\begin{enumerate}
\item x = domain-reliant, there are LTKCs of all ACs other than
those in the domain of $A$ and of all GUs other than those in
  the domain of $G$, i.e.\ in the event
  $\LTKC(\ACs \setminus \dom(A)) \cup \LTKC(\GUs \setminus \dom(G))$.


\item x = GU-domain-reliant, there are LTKCs of all ACs and of
       all GUs other than those in the domain of $G$, i.e.\ in the event
       $\LTKC(\ACs) \cup \LTKC(\GUs \setminus \dom(G))$.

\item x = full, there are LTKCs of all ACs and of all GUs, i.e.\ in the
   event $\LTKC(\ACs) \cup \LTKC(\GUs)$.
\end{enumerate}
\item
We say $T$ guantees \emph{local resilience} when it guarantees at least
domain-reliant resilience.
\end{definition}




==> resil/designs-last.tex <==

\subsubsection{Resilient Designs}

\begin{table}
%\begin{center}
\centering{
\begin{tabular}{|c|c|c||c|c|c|}
\hline
& N & M &  LTKC R. & AL Control & MI R.  \\
\hline \hline 
1 & any & 4/2EV & basic  & yes/no &  ? \\
\hline
2 & any & PC/CR & airport-reliant & no & ?  \\
\hline
3 & $\NGU$ & $M_T$ & full & no &  yes \\ 
\hline
4 & $\NGU$ & $M_T$, 4EV & full & yes & yes\\
\hline 
%5 & $\NOP$ & $M_T$, 4EV & basic & yes & yes\\
%\hline
\end{tabular} }
\vspace*{2ex}
%\end{center} 
\caption{\label{tab:authDesigns} Resilient Authenticated TAGA}
\end{table}

\removed{
Table~\ref{tab:authDesigns} shows how, when using the 
FHMQV\CLS\ as underlying protocol, we obtain secure and resilient
designs for a-TAGA. The table also records the notion of multi-instance 
resiliance inherited 
by the choice of $N$, and whether the crew of the aircraft have
means of checking whether it is indeed a certificate of their
aircraft's domain that will be used by the GU to establish the channel.
We call this `AL Control'.}

%\begin{fact}
%The FHMQV\CLS\ is secure, LTKC resilient, and eav-LTKC resilient
%for a-TAGA.
%\end{fact}


\begin{theorem}
\label{thm:resil}
For $i \in [1,4]$ let $T_i = ($FHMQV\CLS, $N_i, M_i)$ where $N_i$ and $M_i$
are as in Table~\ref{tab:authDesigns}.
For each $i \in [1,5]$, $T_i$ is secure and guarantees the
properties as as shown in row $i$.
\end{theorem}

For our setting designs (3) or (4) are most suitable. In future
work we develop a tool chain to verify its concrete implementation.
%and we
%will develop In future
%work we will develop a tool chain to obtain fully formal tool-assisted
%proofs of the design. 

%best suited when it 
%comes to resilience and flexibity. 

\removed{
However, for other M2M settings 
other combinations might be better. For example, it might be
preferable to establish the key `over the air' and 
secure some safety-critical services by PC/CR/KCM. Based on 
the attack categories and their pre-conditions it is straightforward
to check whether all safety-critical attack states are sufficiently covered.}
%as the Imp2AC direction is not safety-critical, which is not
%necessarily the case in our setting.

%While a-TAGA (1) shows that secure and resilient TAGA is possible without
%channel authenticity (3) and (4) are best suited overall. While




==> resil/designs311.tex <==

\subsection{Resilient Designs}

\begin{table*}
\begin{center}
\begin{tabular}{|c|c|c||c|c|c|c|}
\hline
& N & M &  LTCK Resilience & AL Control (S) & AP Control (S) &
  Multi-Instance R.  \\
\hline \hline 
1 & N-X & PCR & LTKC(GUs$\,\setminus\,$dom(G)) $\cup$ LTKC(ACs) & no & yes & nfc \\
  &     &     & GU-domain-reliant &  & & \\
\hline
2 & N-X & 4/2EV & LTKC(GUs$\,\setminus\,$dom(G) $\cup$ LTKC(ACs$\,\setminus\,$dom(A)) & yes & no & nfc \\
  &     &     & domain-reliant          &  & & \\
\hline
3 & N-GU & Prox & any LTKC  & no & yes & strong\\ 
  &      &      &  fully local  &    &  &\\
\hline
4 & N-GU & Prox, EV & any LTKC  & yes & yes & strong\\
  &      &   EV   &     fully local         &     &  & \\
\hline
\end{tabular}
\end{center} 
\caption{\label{tab:authDesigns} Resilient Authenticated TAGA}
\end{table*}

Table~\ref{tab:authDesigns} shows how we indeed reach the notions of resilience
defined earlier. We have also recorded the notion of
multi-instance resiliance inherited by the choice of $N$,
and a further category  that might be useful in the choice
of a design, explained below: whenever we integrate the   

While (2) is a very lightweight way to obtain resilience 
it only reaches domain-reliant resilience and is dependent
on the human check. The advantage is that when we use the
4EV variant we obtain AP Control for safety-critical
attacks: a safetyc-critical attack state can only be reached
if there is a security incidence in the domain of the
local $A$ (either the crew member doesn't perform the check or
there is a domain LTKC). GU-control is given in all other designs. 
4 eyes check gives the AL conrosl

By choosing the N-GU'model as NFC system we obtain full resilience. Note that
to avoid another (possibly not independent) airport PKI dependency it
is preferable to base this on the GU-bound model rather than a
OP-bound card. By combining it with both 4EV and 4EWalk we can also integrate
AL control. Altogether we obtain:

\begin{theorem}
\label{thm:resil}
Let $P$ be an AKE protocol that is secure and resilient for 
authenticated TAGA, and for $i \in [1,4]$ let $T_i$ be the 
TAGA process defined by $(P, N_i, M_i)$ where $N_i$ and
$M_i$ are defined as shown in Table~\ref{tab:authDesigns}.
Then for each $i \in [1,n]$, $T_i$ guarantees the
properties as as shown in row $i$.
\end{theorem}





==> resil/dual.tex <==
\subsubsection{Property for Dual Control}

When the long-term private keys of both parties are compromised then
the security of implicitly authenticated DH protocols will typically reduce
to that of the basic DH exchange: i.e.\ they will remain secure against
passive attackers based on the secrecy of their ephemeral private keys. 
Note that this is exactly the
property we need to be able to employ an authenticated local channel as a second
line of defense. 

%Authenticated DH protocols will typically maintain the security against
%passive attackers of the unauthenticated DH exchange. 


\removed{
%Finally, we wish that our ... 
if LTKs of both the two entities are compromised then
the secrecy and authentication properties are not affected
as long as the attacker could only eavesdrop into that session.
This means the attacker needs to break channel integrity to
gain sth. In our context, one could say the protocol should
provide at least the g. of the DH exchange even when LTKC. }

\begin{definition}
We say a protocol $P$ guarantees \emph{LTK resilience 
against a passive attacker} if, whenever two parties $G$ and $A$ jointly run 
the protocol, and the attacker has only eavesdropped on
their session (but possibly actively intervenes in other parallel
sessions) then all the secrecy and authentication
guarantees to $A$ and $G$ are given, even when both $A$ and $G$ 
have a LTKC. 
\end{definition}

This property is close to the well-known property of \emph{forward secrecy}
\cite{forwSecr}. Although for practical protocols the two properties will 
typically coincide, in general, they seem incomparable: it seems possible to 
construct an artificial protocol for which the two notions will differ.

\removed{
For practical protocols this property will typically coincide with
the well-known property of forward
secrecy. For practical 
This property is related to but, in general, incomparable to forward 
secrecy.  (appendix?)

\begin{theorem}
TO FORMULATE
Let $(...)$ be taga. if u not compromised ... Then channel
\end{theorem}}


==> resil/general.tex <==

\begin{enumerate}
\item AC control: if such an inc. is safety-critical then in addition
      also in A domain.
\item resilient against scaling: ...
\item resilient against non-domain LTKCs
\end{enumerate}

one domain GU-LTKC and any AC-LTKC ensure resilient against
sufficient: hence, we require that resilient against
parallel scaling:


The later could also be done local
revoked root certificates are updated by a local process, when
     an entity meet somewhere.



==> resil/l14.tex <==
\subsection{Local PKI for Local Service}
When a PKI is to manage the credentials
of an id-indiscriminate service such as TAGA (where an LTKC of 
one party can even impact on the safety of another party) then 
for revocation to be effective two conditions must be met: 
This must be given 
across the various domains of airlines and airports that may
participate in TAGA. 

Most PKIs counter the risk of LTKCs by providing procedures for 
certificate revocation. For revocation to be effective two conditions
must be met: First, LTKCs or security incidences that entail them must 
be detected and the affected certificates revoked before any (wide) 
abuse can take place. Second, verification of a certificate must include 
checking that it has not been revoked via up-to-date revocation lists
or online check. 

Both requirements are impractical in the setting of TAGA:
The first condition underlies the assumption that all airlines
and airports mutually trust each other and apply equivalent security 
management. For example, say airline $U$ of country $\mcU$ and airline 
$R$ of country $\mcR$ both regularly land at airport $M$. 
Then airline $U$ must trust the security of airline $R$'s management of
TAGA credentials as well as that $R$ will never \emph{deliberately} 
hand out TAGA credentials to harm aircraft of $U$ at airport $M$. 
%
The second condition underlies the assumption that when a
GU or AC carry out TAGA pairing they perform an online check
or check a recently updated revocation list (e.g. obtained
at airport). The former requires
Internet connectivity of GUs and ACs themselves, and the latter
connectivity via the that of the airport. 

Both requirements are impractical in the setting of TAGA:
The first condition requires that two airlines that land at the
same airport trust each other's IT security to ensure the required
fast detection and revocation. Moreover, this condition
requires that two airlines, say of two different countries,
that land at the same airport trust each other to not abuse their own
credentials to harm the other. 

Since the setting of TAGA is international  


 to ensure 
a high level of security to
fast detection nd
security  
of security 

all airlines and airports trust
each other to have an (in their view) adequate level of security management 
installed when indeed their security levels can vary considerably.
The first condition also requires that all airlines and airports
trust each other to not abuse a cyber service to harm another
party (e.g.\ by providing an attacker with valid TAGA credentials).
However, the setting of TAGA is international without political
constraints. The second condition   


entities and CA's
participating in TAGA  have a high level of security management 
installed while the security levels of airports and airlines can vary 
considerably. 

but also that they trust each other to not carry out
an insider attack to harm another party (i.e.\ by creating and using a
LTKC in their own domain). However, the setting of TAGA is international 
and 
The second condition requires that TAGA relies on online connectivity
so that the GUs/ACs (perhaps via the airport) can check/obtain the recent 
status of the certificates. 
Hower, the  
TAGA takes place while one of the selling points of TAGA is that it 
does not rely on online connectivity. The second condition

can potentially
lead to them within any participating domain must be detected
quickly and the respective certificates quickly and reliably 

proecudure to be effective two conditions must be met:
First, revocation must be fast and reliable for all 
participating domains. Second, LTKCs of any participating
domain must be detected quickly and reliably so that the respective 
certificate can be revoked before any abuse can take place.

The first condition requires an online revocation procedure
t. an online revocation check whenever
TAGA takes place while one of the selling points of TAGA is that it 
does not rely on online connectivity. The second condition
requires universal trust in all peers and CA's participating in
TAGA to have an adequate level of security management installed
and to never to abuse the service to harm another party.

Since the setting of TAGA is international and the security
levels of airports and airlines can vary considerably
one might prefer not to rely on an assumption of universal trust.

Instead, we advocate the concept of `local PKI for local service'.
It is based on two principles: \emph{local resilience} for the service and
\emph{local responsibility and tracebility} for the PKI. 
The idea behind \emph{local resilience} means that the service
(such as TAGA) is resilient against LTKCs of the domains of
non-local parties. The premise is that this can be ensured
   ensured by local process measures.
if a service is local in that for it to be carried out the participating 
parties come together at one location (such as a parking slot)
then the service can be made resilient against 
non-local LTKCS' by integrating local process measures into the security design.
Local measures can e.g.\ comprise visual monitoring by local staff 
(such as GU operators and crew), detection measures built into
the physical entities, local staff reacting to security alerts,
and local channels established by local equipment and staff. 
Hence, two
parties only need to trust each others security management when
they ``touch locally" for the service. 

\begin{table}
\input{resil/tab-localPKI}
\caption{\label{t:localPKI} }
\end{table}

This then ensures that the \emph{PKI} is based on.
\emph{Local responsibility and traceability}: means that every domain 
(e.g.\ every airline and airport participating in TAGA) is responsible 
for managing the keys and certificates of their domain, and that
if a security incidence happens due to a LTKC this can be
traced back to the domain responsible. In particular, this
includes the requirements listed in Table~\ref{t:localPKI}.
\footnote{Note that this does no exclude that several domains
jointly commission a central authority to manage this; but it will
allow that there is a central authority for only part of the TAGA
participants.}

We now make precise notions of local resilience for TAGA. 
Then, in the remainder of the section, we explore how 
these notions of resilience can be reached by a combination of 
advanced properties of the underlying AKE protocol and local 
process measures.

\begin{definition}
Let $T$ be an authenticated TAGA process.
\item
We say $T$ guarantees \emph{$x$ resilience}, where 
\emph{$x = \{$domain-reliant, GU-domain-reliant, full$\}$}, 
if, whenever a ground service that integrates $T$ takes place 
at a location $L$ between AC $A$ and GU $G$ (G1, Gn) then
$T$ guarantees Secure TAGA II to $A$ and $G$ even when, for 
\begin{enumerate}
\item x = domain-reliant, there are LTKCs of all ACs other than 
those in the domain of $A$ and of all GUs other than those in 
  the domain of $G$, i.e.\ in the event 
  $\LTKC(\ACs \setminus \dom(A)) \cup \LTKC(\GUs \setminus \dom(G))$.
  

\item x = GU-domain-reliant, there are LTKCs of all ACs and of
       all GUs other than those in the domain of $G$, i.e.\ in the event
       $\LTKC(\ACs) \cup \LTKC(\GUs \setminus \dom(G))$.

\item x = full, there are LTKCs of all ACs and of all GUs, i.e.\ in the
   event $\LTKC(\ACs) \cup \LTKC(\GUs)$.
\end{enumerate}
\item
We say $T$ guantees local resilience/
is suitably resilient for local PKI when it guarantees at least
domain-reliant resilience. 
\end{definition}


Domain-reliant resilience ensures that an airline $\mcA$ must only 
trust an airport $\mcH$'s key management processes when ACs governed 
by $\mcA$ land at $\mcH$ rather than any airport participating in TAGA, 
and analogously for the other direction. GU-domain-reliant resilience 
is stronger in that an airport does not require to trust 
the airline's key management processes at all. 
Full resilience ensures that TAGA has a second line of
defense and does not rely on certificates as long as the local measures
work. We now show how such resiliance can be achieved by a combination
of advanced properties of the underlying AKE protocol and
local process measures. 

the airport this
 only "locally touching
parties" need mutually trust each other. The premise is that
then there is already trust.
And similarly the other way around.
But it will
be unaffected by any other airport's security even when they
also participate in TAGA. 



%  as an indpendent /dual control/ GU-Op not compr. and card okay
% local card better./as long as GU-Op not compromised and local card okay.


==> resil/local-PKI-save.tex <==
\subsection{Local PKI}

In a setting such as TAGA where the service is
id-indiscriminate 
(certificate is more about authorization)
an LTKC  any AC party  can impact on another peer.
a fast revocation process is necessary. This is impractical
in this setting for two reasons:
One is that TAGA should not depend on online connection as necessary
for an online revocation check (such as).
The second is that TAGA spans parties of an international,a
that cannot be  
and how can we trust each airport that wishes to 
a revocation process   to be reliably be implemented
even if a central authority is commissioned to do so, it will
depend on the local entities to report on local domains compromises in their
domain. it seems

Instead, we advocate the principle of \emph{Local PKI} for TAGA:
local responsibility and resilience against compromise in other domains:
\begin{enumerate}
\item Every party is responsible for managing their own certificates:
\begin{enumerate}
\item they only use private keys and corresponding certificates
      that to their knowledge are secure. 
\item if some incidence happens and involves a certificate of their
      domain then they deal with. traceable cause
\item revoked root certificates are updated by a local process, when
     an entity meet somewhere.   
\item the process itself is resilient against ..
\end{enumerate}
\end{enumerate} 
and scalability.

\begin{enumerate}
\item if an incidence happens at $L$ then compromise/sec. violation 
      within domain of $L$.   (or A)
\item AC control: if such an inc. is safety-critical then in addition
      also in A domain. 
\item resilient against scaling: ... 
\item resilient against non-domain LTKCs
\end{enumerate}


LTKC-AC.d combine with detection measures.
detection measures, monitoring of local staff.
and local measures such as staff reacting to security alerts,
etc. lcoal channel ground staff/crew

\input{resil/local}

%            as an indpendent /dual control/ GU-Op not compr. and card okay
% local card better./as long as GU-Op not compromised and local card okay.

one domain GU-LTKC and any AC-LTKC ensure resilient against
sufficient: hence, we require that resilient against
parallel scaling:

and sequential: against any AC in sequence: third.
or many parked.


to reach MitM resilient against AC-LTKC-GU(S) or AC-LTKC-AC

one G against different AC.

resilient against LTKC-GU up to 

TAGA takes place at $L$. locally resilient if
say a 

if the AC is involved in key establsihing then /the attack then
mitm. then secure up to LTKC-GU (S)


==> resil/local-PKIsave3.tex <==
\subsection{Local PKI for Local Service}

Most PKIs counter the risk of LTKCs by providing procedures for 
certificate revocation. When a PKI is to manage the credentials
of an id-indiscriminate service such as  
TAGA (where an LTKC of one party can impact on
the safety of another party) then for a revocation
proecudure to be effective two conditions must be met:
First, revocation must be fast and reliable for all 
participating domains. Second, LTKCs of any participating
domain must be detected quickly and reliably so that the respective 
certificate can be revoked before any abuse can take place.

Both requirements are impractical in the setting of TAGA:
The first condition requires an online revocation check whenever
TAGA takes place while one of the selling points of TAGA is that it 
does not rely on online connectivity. The second condition
requires universal trust in all peers and CA's participating in
TAGA to have an adequate level of security management installed
and to never to abuse the service to harm another party.
Since the setting of TAGA is international and the security
levels of airports and airlines can vary considerably
one might prefer not to rely on an assumption of universal trust.

Instead, we advocate the concept of `local PKI for local service'.
It is based on two principles: \emph{local resilience} for the service and
\emph{local responsibility and tracebility} for the PKI. 
The idea behind \emph{local resilience} means that the service
(such as TAGA) is resilient against LTKCs of the domains of
non-local parties. The premise is that this can be ensured
   ensured by local process measures.
if a service is local in that for it to be carried out the participating 
parties come together at one location (such as a parking slot)
then the service can be made resilient against 
non-local LTKCS' by integrating local process measures into the security design.
Local measures can e.g.\ comprise visual monitoring by local staff 
(such as GU operators and crew), detection measures built into
the physical entities, local staff reacting to security alerts,
and local channels established by local equipment and staff. 
Hence, two
parties only need to trust each others security management when
they ``touch locally" for the service. 

\begin{table}
\input{resil/tab-localPKI}
\caption{\label{t:localPKI} }
\end{table}

This then ensures that the \emph{PKI} is based on.
\emph{Local responsibility and traceability}: means that every domain 
(e.g.\ every airline and airport participating in TAGA) is responsible 
for managing the keys and certificates of their domain, and that
if a security incidence happens due to a LTKC this can be
traced back to the domain responsible. In particular, this
includes the requirements listed in Table~\ref{t:localPKI}.
\footnote{Note that this does no exclude that several domains
jointly commission a central authority to manage this; but it will
allow that there is a central authority for only part of the TAGA
participants.}

We now make precise notions of local resilience for TAGA. 
Then, in the remainder of the section, we explore how 
these notions of resilience can be reached by a combination of 
advanced properties of the underlying AKE protocol and local 
process measures.

\begin{definition}
Let $T$ be an authenticated TAGA process.
\item
We say $T$ guarantees \emph{$x$ resilience}, where 
\emph{$x = \{$domain-reliant, GU-domain-reliant, full$\}$}, 
if, whenever a ground service that integrates $T$ takes place 
at a location $L$ between AC $A$ and GU $G$ (G1, Gn) then
$T$ guarantees Secure TAGA II to $A$ and $G$ even when, for 
\begin{enumerate}
\item x = domain-reliant, there are LTKCs of all ACs other than 
those in the domain of $A$ and of all GUs other than those in 
  the domain of $G$, i.e.\ in the event 
  $\LTKC(\ACs \setminus \dom(A)) \cup \LTKC(\GUs \setminus \dom(G))$.
  

\item x = GU-domain-reliant, there are LTKCs of all ACs and of
       all GUs other than those in the domain of $G$, i.e.\ in the event
       $\LTKC(\ACs) \cup \LTKC(\GUs \setminus \dom(G))$.

\item x = full, there are LTKCs of all ACs and of all GUs, i.e.\ in the
   event $\LTKC(\ACs) \cup \LTKC(\GUs)$.
\end{enumerate}
\item
We say $T$ guantees local resilience/
is suitably resilient for local PKI when it guarantees at least
domain-reliant resilience. 
\end{definition}


Domain-reliant resilience ensures that an airline $\mcA$ must only 
trust an airport $\mcH$'s key management processes when ACs governed 
by $\mcA$ land at $\mcH$ rather than any airport participating in TAGA, 
and analogously for the other direction. GU-domain-reliant resilience 
is stronger in that an airport does not require to trust 
the airline's key management processes at all. 
Full resilience ensures that TAGA has a second line of
defense and does not rely on certificates as long as the local measures
work. We now show how such resiliance can be achieved by a combination
of advanced properties of the underlying AKE protocol and
local process measures. 

the airport this
 only "locally touching
parties" need mutually trust each other. The premise is that
then there is already trust.
And similarly the other way around.
But it will
be unaffected by any other airport's security even when they
also participate in TAGA. 



%  as an indpendent /dual control/ GU-Op not compr. and card okay
% local card better./as long as GU-Op not compromised and local card okay.


==> resil/local.tex <==

%\newcommand{\LTKC}{\mathit{LTKC}}
\newcommand{\dom}{\mathit{dom}}
\newcommand{\nonDom}{\neg \dom}
\newcommand{\ACs}{\mathit{ACs}}
%\newcommand{\GUs}{\mathit{GUs}}

\begin{definition}
We say $T$ guarantees \emph{$X$ Resilience}, where 
\emph{$x = \{$domain-reliant, GU-domain-reliant, full$\}$}, 
if, whenever a ground service with TAGA takes place at a location
$L$ between AC $A$ and GU $G$ (G1, Gn) then
$T$ guarantees Secure TAGA II to $A$ and $G$ even when, if 
\begin{enumerate}
\item x = domain-reliant, there are LTKCs of all ACs other than 
those in the domain of $A$ and of all GUs other than those in 
  the domain of $G$, i.e.\ in the event 
  $\LTKC(\ACs \setminus \dom(A)) \cup \LTKC(\GUs \setminus \dom(G))$.
  

\item x = GU-domain-reliant, there are LTKCs of all ACs and of
       all GUs other than those in the domain of $G$, i.e.\ in the event
       $\LTKC(\ACs) \cup \LTKC(\GUs \setminus \dom(G))$.

\item x = full, there are LTKCs of all ACs and of all GUs, i.e.\ in the
   event $\LTKC(\ACs) \cup \LTKC(\GUs)$.
\end{enumerate}

We say $T$ is suitable for local PKI when it guarantees at least
domain-reliant resilience. 
\end{definition}



==> resil/localPKI-save2.tex <==
\subsection{Local PKI for Local Service}

In a setting such as TAGA where the service is id-indiscriminate
and LTKC of a party $A$ can impact on the safety of another peer $B$
when using a traditional PKI based on revocation of certificates two 
things must be given: First, a fast and reliable revocation process
must be in place. Second, there must be trust that LTKCs are
detected quickly so that the certifcates can be revoked before
abuse has already happend. 

Both requirements are impractical in the setting of TAGA:
The first point requires online revocation check connection of all parties 
while one of the selling points of TAGA is that it works 
independent on online connectivity. 
The second point requires that there is trust  
This requires that the parties trust
all peers and CA's to adequate level of security management and
non-insider attacks in place. E.g. if HSMs are used for peer
 in trust in peers to not meddle with their HSMs, and the CAs
to ..detect security compromises.
each other or a central party's  to detect security compromises.
Since the setting of TAGA is international and
the security levels between airports and airlines can vary considerably
one might wish to not rely on this.cerntral/peer trust.

This is why for authenticated TAGA we advocate the concept of 
\emph{local PKI}: 

and how can we trust each airport that wishes to 
a revocation process   to be reliably be implemented
even if a central authority is commissioned to do so, it will
depend on the local entities to report on local domains compromises in their
domain. it seems

Instead, we advocate the principle of \emph{Local PKI} for TAGA:
It is based on two principles: \emph{local responsibility and
traceability} and \emph{local resilience}. 

\begin{table}
\input{resil/tab-localPKI}
\caption{\label{t:localPKI} }
\end{table}

Local responsibility and traceability means that every domain 
(e.g.\ every airline and airport participating in TAGA) is responsible 
for managing the keys and certificates of their domain, and that
if a security incidence happens due to a LTKC this can be
traced back to the domain responsible. In particular, this
includes the requirements listed in Table~\ref{t:localPKI}.
\footnote{Note that this does no exclude that several domains
jointly commission a central authority to manage this; but it will
allow that there is a central authority for only part of the TAGA
participants.}

\emph{Local resilience} means that the service (e.g.\ TAGA process) 
itself is resilient against LTKCs of the domains of non-local parties. 
Hence, two
parties only need to trust each others security management when
they ``touch locally" for the service. For TAGA we define this as follows:
   ensured by local process measures.

\input{resil/local}

Domain-reliant resilience ensures that an airline $\mcH$ must only 
trust an airport $\mcG$'s lt key management processes when 
it decides to land there rather
than any airport participating in TAGA, and analogously for the
other direction. GU-domain-reliant resilience is stronger in that
it does not require to trust the airline's key management processes
at all. Full resilience ensures that TAGA has a second line of
defense and does not rely on certificates. 
We now show how such resiliance can be achieved by a combination
of advanced properties of the underlying AKE protocol and
local process measures. (such as monitoring by local ground staff/
crew, reacting to security alerts, detection measures built into
the local physical entities, local channel established by 
local equipment and staff). 

the airport this
 only "locally touching
parties" need mutually trust each other. The premise is that
then there is already trust.
And similarly the other way around.
But it will
be unaffected by any other airport's security even when they
also participate in TAGA. 



%  as an indpendent /dual control/ GU-Op not compr. and card okay
% local card better./as long as GU-Op not compromised and local card okay.


==> resil/localPKI.tex <==
\subsection{Local PKI for Local Service}
%across the various domains of airlines and airports that may
%participate in TAGA. 

Most PKIs counter the risk of LTKCs by providing procedures for 
certificate revocation. For revocation to be effective two conditions
must be met: First, LTKCs or security incidences that entail them must 
be detected and the affected certificates revoked before any unacceptable 
damage can occur. Second, verification of a certificate must include 
checking that it has not been revoked. This can either be based on
an online certificate status check: the end entity queries the CA as to
whether the certificate is valid; or on certificate revocation lists
(CRL): the end entity checks that the certificate does not appear
on the CA's CRL, where CRLs must be given out by each CA and 
retrieved by the end entities in a timely manner.
In both cases it must be ensured that in the gap between certificate
revocation and the time when the certifcate becomes invalid at the
end points no unacceptable damage can occur. 

Both requirements are impractical in the setting of TAGA.
The first condition underlies the assumption that all airlines
and airports mutually trust each other and apply equivalent security 
management. For example, say airline $U$ of country $\mcU$ and airline 
$R$ of country $\mcR$ both regularly land at airport $M$. Then airline 
$U$ must trust the security of airline $R$'s management of
TAGA credentials as well as that $R$ will never \emph{deliberately}
hand out TAGA credentials to harm aircraft of $U$ at airport $M$. 
Otherwise Attack~\ref{} is possible.
The second condition brings about dependency of TAGA pairing on
Internet connectivity.  When a GU or AC verify their peer's 
certificate during TAGA they must either perform an online check
or they must obtain the current CRL from the airport, which in turn
needs Internet connectiviy to keep them up-to-date.
However, one of the main selling points of TAGA is that it does
not rely on online connectivity.

Instead, we can make use of the locality of the setting: Whenever 
two TAGA parties wish to mutually authenticate themselves based
on their long-term credentials they are never remote but proximate:
they are located at the same parking slot. On the one hand,
this motivates a notion of local resilience against LTKC:
while local parties must mutually trust each other and their 
security domains, we require that they should never be affected by 
a security incidence in key managament infrastructures of another 
airline or airport. On the other hand, the locality of the setting
also provides means to achieve this (and stronger) notions of
LTKC resilience: we can harden TAGA against LTKCs 
by local process measures. This can involve visual monitoring by local staff 
(such as GU operators and crew), detection measures built into
the physical entities, local staff reacting to security alerts,
and local channels established by local equipment and staff (such as
the TAGA transport). 




TAGA should be resilient against LTKCs in that each party
should depend at most on the key instrastructure  




Instead, we advocate the concept of `local PKI for local service'.
It is possible in a setting like TAGA where:
whenever two entities authenticate themselves
anhcored in the PKI then they are indeed at the same location/locally proximate.



It is based on two principles: \emph{local resilience} for the service and
\emph{local responsibility and tracebility} for the PKI. 

\paragraph*{Local resilience}


The idea behind \emph{local resilience} means that the service
(such as TAGA) is resilient against LTKCs of the domains of
non-local parties. The premise is that this can be ensured
   ensured by local process measures.
if a service is local in that for it to be carried out the participating 
parties come together at one location (such as a parking slot)
then the service can be made resilient against 
non-local LTKCS' by integrating local process measures into the security design.
Local measures can e.g.\ comprise

Hence, two
parties only need to trust each others security management when
they ``touch locally" for the service. 

\begin{table}
\input{resil/tab-localPKI}
\caption{\label{t:localPKI} }
\end{table}

This then ensures that the \emph{PKI} is based on.
\emph{Local responsibility and traceability}: means that every domain 
(e.g.\ every airline and airport participating in TAGA) is responsible 
for managing the keys and certificates of their domain, and that
if a security incidence happens due to a LTKC this can be
traced back to the domain responsible. In particular, this
includes the requirements listed in Table~\ref{t:localPKI}.
\footnote{Note that this does no exclude that several domains
jointly commission a central authority to manage this; but it will
allow that there is a central authority for only part of the TAGA
participants.}

We now make precise notions of local resilience for TAGA. 
Then, in the remainder of the section, we explore how 
these notions of resilience can be reached by a combination of 
advanced properties of the underlying AKE protocol and local 
process measures.

\begin{definition}
Let $T$ be an authenticated TAGA process.
\item
We say $T$ guarantees \emph{$x$ resilience}, where 
\emph{$x = \{$domain-reliant, GU-domain-reliant, full$\}$}, 
if, whenever a ground service that integrates $T$ takes place 
at a location $L$ between AC $A$ and GU $G$ (G1, Gn) then
$T$ guarantees Secure TAGA II to $A$ and $G$ even when, for 
\begin{enumerate}
\item x = domain-reliant, there are LTKCs of all ACs other than 
those in the domain of $A$ and of all GUs other than those in 
  the domain of $G$, i.e.\ in the event 
  $\LTKC(\ACs \setminus \dom(A)) \cup \LTKC(\GUs \setminus \dom(G))$.
  

\item x = GU-domain-reliant, there are LTKCs of all ACs and of
       all GUs other than those in the domain of $G$, i.e.\ in the event
       $\LTKC(\ACs) \cup \LTKC(\GUs \setminus \dom(G))$.

\item x = full, there are LTKCs of all ACs and of all GUs, i.e.\ in the
   event $\LTKC(\ACs) \cup \LTKC(\GUs)$.
\end{enumerate}
\item
We say $T$ guantees local resilience/
is suitably resilient for local PKI when it guarantees at least
domain-reliant resilience. 
\end{definition}


Domain-reliant resilience ensures that an airline $\mcA$ must only 
trust an airport $\mcH$'s key management processes when ACs governed 
by $\mcA$ land at $\mcH$ rather than any airport participating in TAGA, 
and analogously for the other direction. GU-domain-reliant resilience 
is stronger in that an airport does not require to trust 
the airline's key management processes at all. 
Full resilience ensures that TAGA has a second line of
defense and does not rely on certificates as long as the local measures
work. We now show how such resiliance can be achieved by a combination
of advanced properties of the underlying AKE protocol and
local process measures. 

the airport this
 only "locally touching
parties" need mutually trust each other. The premise is that
then there is already trust.
And similarly the other way around.
But it will
be unaffected by any other airport's security even when they
also participate in TAGA. 



%  as an indpendent /dual control/ GU-Op not compr. and card okay
% local card better./as long as GU-Op not compromised and local card okay.


==> resil/localResil-long.tex <==
\subsection{Motivation and Concept}
%across the various domains of airlines and airports that may
%participate in TAGA. 

Most PKIs counter the risk of LTKCs by providing procedures for 
certificate revocation. For revocation to be effective two conditions
must be met: First, LTKCs or security incidences that entail them must 
be detected and the affected certificates revoked before any unacceptable 
damage can occur. Second, verification of a certificate must include 
checking that it has not been revoked. This can either be based on
an online certificate status check: the end entity queries the CA as to
whether the certificate is valid; or on certificate revocation lists
(CRL): the end entity checks that the certificate does not appear
on the CA's CRL, where CRLs must be given out by each CA and 
retrieved by the end entities in a timely manner.
In both cases it must be ensured that in the gap between certificate
revocation and the time when the certifcate becomes invalid at the
end points no unacceptable damage can occur. 

Both requirements are impractical in the setting of TAGA.
The first condition underlies the assumption that all airlines
and airports mutually trust each other and apply equivalent security 
management. For example, say airline $U$ of country $\mcU$ and airline 
$R$ of country $\mcR$ both regularly land at airport $M$. Then airline 
$U$ must trust the security of airline $R$'s management of
TAGA credentials as well as that $R$ will never \emph{deliberately}
hand out TAGA credentials to harm aircraft of $U$ at airport $M$. 
Otherwise Attack~\ref{} is possible.
The second condition brings about dependency of TAGA pairing on
Internet connectivity.  When a GU or AC verify their peer's 
certificate during TAGA they must either perform an online check
or they must obtain the current CRL from the airport, which in turn
needs Internet connectiviy to keep them up-to-date.
However, one of the main selling points of TAGA is that it does
not rely on online connectivity.

Instead, we can make use of the locality of the setting: Whenever 
two TAGA parties wish to mutually authenticate themselves based
on their long-term credentials they are never remote but proximate:
they are located at the same parking slot. On the one hand,
this motivates a notion of local resilience against LTKC:
while local parties must mutually trust each other and their 
security domains, we require that they should never be affected by 
a security incidence in key managament infrastructures of another 
airline or airport. On the other hand, the locality of the setting
also provides means to achieve this (and stronger) notions of
LTKC resilience: we can harden TAGA against LTKCs 
by local process measures. This can involve visual monitoring by local staff 
(such as GU operators and crew), detection measures built into
the physical entities, local staff reacting to security alerts,
and local channels established by local equipment and staff (such as
the TAGA transport). 

%We now make precise notions of local resilience for TAGA. 
%Then, in the remainder of the section, we explore how 
%these notions of resilience can be reached by a combination of 
%advanced properties of the underlying AKE protocol and local 
%process measures.

\begin{definition}
Let $T$ be an authenticated TAGA process.
\item
We say $T$ guarantees \emph{$x$ resilience}, where 
\emph{$x = \{$domain-reliant, GU-domain-reliant, full$\}$}, 
if, whenever a ground service that integrates $T$ takes place 
at a location $L$ between AC $A$ and GU $G$ (G1, Gn) then
$T$ guarantees Secure TAGA II to $A$ and $G$ even when, for 
\begin{enumerate}
\item x = domain-reliant, there are LTKCs of all ACs other than 
those in the domain of $A$ and of all GUs other than those in 
  the domain of $G$, i.e.\ in the event 
  $\LTKC(\ACs \setminus \dom(A)) \cup \LTKC(\GUs \setminus \dom(G))$.
  

\item x = GU-domain-reliant, there are LTKCs of all ACs and of
       all GUs other than those in the domain of $G$, i.e.\ in the event
       $\LTKC(\ACs) \cup \LTKC(\GUs \setminus \dom(G))$.

\item x = full, there are LTKCs of all ACs and of all GUs, i.e.\ in the
   event $\LTKC(\ACs) \cup \LTKC(\GUs)$.
\end{enumerate}
\item
We say $T$ guantees local resilience/
is suitably resilient for local PKI when it guarantees at least
domain-reliant resilience. 
\end{definition}


Domain-reliant resilience ensures that an airline $\mcA$ must only 
trust an airport $\mcH$'s key management processes when ACs governed 
by $\mcA$ land at $\mcH$ rather than any airport participating in TAGA, 
and analogously for the other direction. GU-domain-reliant resilience 
is stronger in that an airport does not require to trust 
the airline's key management processes at all. 
Full resilience ensures that TAGA has a second line of
defense and does not rely on certificates as long as the local measures
work. We now show how such resiliance can be achieved by a combination
of advanced properties of the underlying AKE protocol and
local process measures. 

the airport this
 only "locally touching
parties" need mutually trust each other. The premise is that
then there is already trust.
And similarly the other way around.
But it will
be unaffected by any other airport's security even when they
also participate in TAGA. 



%  as an indpendent /dual control/ GU-Op not compr. and card okay
% local card better./as long as GU-Op not compromised and local card okay.


==> resil/localResil311.tex <==
\paragraph*{Motivation and Concept}
%across the various domains of airlines and airports that may
%participate in TAGA. 

Most PKIs counter the risk of LTKCs by providing procedures for 
certificate revocation. For revocation to be effective two conditions
must be met: First, LTKCs or security incidences that entail them must 
be detected and the affected certificates revoked before any unacceptable 
damage can occur. Second, verification of a certificate must include 
checking that it has not been revoked. This can either be based on
an online check of the certificate status, %(the end entity queries
%the CA as to whether the certificate is valid), 
or on certificate revocation lists (CRLs), which must be given out by 
the CAs and retrieved by the end entities in a timely manner.

\removed{
 : the end entity queries the CA as to
whether the certificate is valid; or 
(CRL): the end entity checks that the certificate does not appear
on the CA's CRL, where CRLs must be given out by each CA and 
retrieved by the end entities in a timely manner.
In both cases it must be ensured that in the gap between certificate
revocation and the time when the certifcate becomes invalid at the
end points no unacceptable damage can occur. }

Both requirements are impractical in the setting of TAGA.
The first condition underlies the assumption that all airlines
and airports mutually trust each other and apply equivalent security 
management. 
\removed{
For example, say airline $U$ of country $\mcU$ and airline 
$R$ of country $\mcR$ both regularly land at airport $M$. Then airline 
$U$ must trust the security of airline $R$'s management of
TAGA credentials as well as that $R$ will never \emph{deliberately}
hand out TAGA credentials to harm aircraft of $U$ at airport $M$. 
Otherwise Attack~\ref{} is possible.}
The second condition brings about dependency of TAGA on
Internet connectivity: When a GU or AC verify their peer's 
certificate during TAGA they must either perform an online check
or they must obtain the current CRL from the airport, which in turn
requires Internet connectiviy to keep the CRLs up-to-date.
%However, one of the main selling points of TAGA is that it does
%not rely on online connectivity.

Instead, we can make use of the locality of the setting: Whenever 
two TAGA parties wish to mutually authenticate themselves based
on their long-term credentials they are located at the same parking 
slot. This motivates TAGA should guarantee 
resilience against non-local LTKCs in the following sense: 
While local TAGA parties must mutually trust each other 
and their security domains, they should never be affected by 
a security incidence in the key management processes of another
airline or airport. Moreover, the locality of the setting
also provides means to achieve this (and stronger) notions of
local resilience since we can include local process measures into
the security design. 

\removed{
\begin{definition}
Let $T$ be a TAGA process that guarantees secure TAGA II.
We say $T$ guarantees \emph{basic LTKC resilience}
if, whenever an instance of $T$ is carried out between a
GU $G$ and an AC $A$ at a parking slot $L$ then $T$ guarantees
secure TAGA II to $G$ and $A$ even when all ACs and GUs other than those
in the domain of $A$ and $G$ have a LTKC.
\end{definition}}

\removed{
For example,
this can involve measures such as visual monitoring by local 
GU operators and crew, physical detection measures built into
the local GU and AC, or second line of defense by a local channel 
established by local equipment and staff.}

%We now make precise notions of local resilience for TAGA. 
%Then, in the remainder of the section, we explore how 
%these notions of resilience can be reached by a combination of 
%advanced properties of the underlying AKE protocol and local 
%process measures.

\begin{definition}
Let $T$ be an authenticated TAGA process that guarantees
secure TAGA II.
We say $T$ guarantees \emph{$x$ LTKC resilience}, where 
\emph{$x = \{$basic, airport-reliant, full$\}$}, 
if, whenever an instance of $T$ is carried out between
a GU $G$ and an AC $A$ at a parking slot $L$ then
$T$ guarantees Secure TAGA II to $G$ and $A$ even when, 
\begin{enumerate}
\item for \emph{x = basic,} all ACs and GUs other than
those in the domain of $A$ and $G$ have a LTKC.
\item for \emph{x = airport-reliant,} all ACs and all GUs other
 than those in the domain of $G$ have a LTKC.
 \item for \emph{x = full,} all ACs and GUs have a LTKC. 
\end{enumerate}
\end{definition}

\emph{Domain-reliant resilience} ensures that an airline $\mcA$ must 
only trust the key management processes of airports where its ACs
land (rather than other airports or other airlines participating
in TAGA), and analogously for the other direction. 
\emph{GU-domain-reliant resilience} is stronger in that an airport 
does not require to trust the airline's key management processes at all. 
\emph{Full resilience} ensures that TAGA has a second line of
defense and does not rely on long-term credentials as long as the local
measures are not compromised.  

\input{resil/resil-basic}
\input{resil/resil-ac}
\input{resil/resil-full}

\removed{
We now show how such resiliance can be achieved by a combination
of advanced properties of the underlying AKE protocol and
local process measures. 

the airport this
 only "locally touching
parties" need mutually trust each other. The premise is that
then there is already trust.
And similarly the other way around.
But it will
be unaffected by any other airport's security even when they
also participate in TAGA. 
}


%  as an indpendent /dual control/ GU-Op not compr. and card okay
% local card better./as long as GU-Op not compromised and local card okay.


==> resil/localResildef.tex <==
\paragraph*{Motivation and Concept}
%across the various domains of airlines and airports that may
%participate in TAGA. 

Most PKIs counter the risk of LTKCs by providing procedures for 
certificate revocation. For revocation to be effective two conditions
must be met: First, LTKCs or security incidences that entail them must 
be detected and the affected certificates revoked before any unacceptable 
damage can occur. Second, verification of a certificate must include 
checking that it has not been revoked. This can either be based on
an online check of the certificate status, %(the end entity queries
%the CA as to whether the certificate is valid), 
or on certificate revocation lists (CRLs), which must be given out by 
the CAs and retrieved by the end entities in a timely manner.

\removed{
 : the end entity queries the CA as to
whether the certificate is valid; or 
(CRL): the end entity checks that the certificate does not appear
on the CA's CRL, where CRLs must be given out by each CA and 
retrieved by the end entities in a timely manner.
In both cases it must be ensured that in the gap between certificate
revocation and the time when the certifcate becomes invalid at the
end points no unacceptable damage can occur. }

Both requirements are impractical in the setting of TAGA.
The first condition underlies the assumption that all airlines
and airports mutually trust each other and apply equivalent security 
management. 
\removed{
For example, say airline $U$ of country $\mcU$ and airline 
$R$ of country $\mcR$ both regularly land at airport $M$. Then airline 
$U$ must trust the security of airline $R$'s management of
TAGA credentials as well as that $R$ will never \emph{deliberately}
hand out TAGA credentials to harm aircraft of $U$ at airport $M$. 
Otherwise Attack~\ref{} is possible.}
The second condition brings about dependency of TAGA on
Internet connectivity: When a GU or AC verify their peer's 
certificate during TAGA they must either perform an online check
or they must obtain the current CRL from the airport, which in turn
requires Internet connectiviy to keep the CRLs up-to-date.
%However, one of the main selling points of TAGA is that it does
%not rely on online connectivity.

Instead, we can make use of the locality of the setting: Whenever 
two TAGA parties wish to mutually authenticate themselves based
on their long-term credentials they are located at the same parking 
slot. This motivates TAGA should guarantee 
resilience against non-local LTKCs in the following sense: 
While local TAGA parties must mutually trust each other 
and their security domains, they should never be affected by 
a security incidence in the key management processes of another
airline or airport. Moreover, the locality of the setting
also provides means to achieve this (and stronger) notions of
local resilience since we can include local process measures into
the security design. 

\begin{definition}
Let $T$ be a TAGA process that guarantees secure TAGA II.
We say $T$ guarantees \emph{basic LTKC resilience}
if, whenever an instance of $T$ is carried out between a
GU $G$ and an AC $A$ at a parking slot $L$ then $T$ guarantees
secure TAGA II to $G$ and $A$ even when all ACs and GUs other than those
in the domain of $A$ and $G$ have a LTKC.
\end{definition}


\removed{
For example,
this can involve measures such as visual monitoring by local 
GU operators and crew, physical detection measures built into
the local GU and AC, or second line of defense by a local channel 
established by local equipment and staff.}

%We now make precise notions of local resilience for TAGA. 
%Then, in the remainder of the section, we explore how 
%these notions of resilience can be reached by a combination of 
%advanced properties of the underlying AKE protocol and local 
%process measures.

\begin{definition}
Let $T$ be an authenticated TAGA process that guarantees
secure TAGA II.
We say $T$ guarantees \emph{$x$ LTKC resilience}, where 
\emph{$x = \{$basic, airport-reliant, full$\}$}, 
if, whenever an instance of $T$ is carried out between
a GU $G$ and an AC $A$ at a parking slot $L$ then
$T$ guarantees Secure TAGA II to $G$ and $A$ even when, 
\begin{enumerate}
\item for \emph{x = domain-reliant,} all ACs and GUs other than
those in the domain of $A$ and $G$ have a LTKC.

there are LTKCs of all ACs other than 
those in the domain of $A$ and of all GUs other than those in 
  the domain of $G$, i.e.\ in the event 
  $\LTKC(\ACs \setminus \dom(A)) \cup \LTKC(\GUs \setminus \dom(G))$.
  

\item \emph{x = GU-domain-reliant,} there are LTKCs of all ACs and of
       all GUs other than those in the domain of $G$, i.e.\ in the event
       $\LTKC(\ACs) \cup \LTKC(\GUs \setminus \dom(G))$.

\item \emph{x = full local,} there are LTKCs of all ACs and of all 
   GUs, i.e.\ in the
   event $\LTKC(\ACs) \cup \LTKC(\GUs)$.
\end{enumerate}
\item
We say $T$ guarantees \emph{local resilience} when it guarantees at least
domain-reliant resilience. 
\end{definition}

\emph{Domain-reliant resilience} ensures that an airline $\mcA$ must 
only trust the key management processes of airports where its ACs
land (rather than other airports or other airlines participating
in TAGA), and analogously for the other direction. 
\emph{GU-domain-reliant resilience} is stronger in that an airport 
does not require to trust the airline's key management processes at all. 
\emph{Full resilience} ensures that TAGA has a second line of
defense and does not rely on long-term credentials as long as the local
measures are not compromised.  

\input{resil/resil-basic}
\input{resil/resil-ac}
\input{resil/way-channel}

\removed{
We now show how such resiliance can be achieved by a combination
of advanced properties of the underlying AKE protocol and
local process measures. 

the airport this
 only "locally touching
parties" need mutually trust each other. The premise is that
then there is already trust.
And similarly the other way around.
But it will
be unaffected by any other airport's security even when they
also participate in TAGA. 
}


%  as an indpendent /dual control/ GU-Op not compr. and card okay
% local card better./as long as GU-Op not compromised and local card okay.


==> resil/measure-human.tex <==
\begin{figure}
\input{figures/fig-measure-human}
\caption{\label{fig:meas:human} Last NFC tap extended 
by human verification of AC}
\end{figure}

\subsubsection{Human Verification of AC}

The first measure makes use of the awareness of the GU operator: 
while the GU has no means to verify that the received AC certificate 
(and information therein) belongs to the AC present at the parking 
position, clearly, the GU operator has sight of the AC. Hence, 
she is able to verify that visually observable features of the AC 
such as its type and airline agree with the information 
received by the GU. 
%The TAGA process only needs to be extended by
%integrating a step of human verification after the final NFC tap:
   

\begin{measure}[`Two Eyes' Verification of AC (2EV)]
\label{m:human:two}
We assume the TAGA controller of the GU is equipped with a display and
two input buttons: one to confirm, and the second to stop the 
process and raise an alarm. Then the last NFC tap can be extended by
human verification as illustrated in Fig.~\ref{fig:meas:human}. First, 
the operator transfers the second message by NFC tap to the 
GU's controller as usual. Recall that this message contains an AC certificate
$\cert_\mcA(A, W_A, T_A, V_A)$, where $\mcA$ is the airline of $A$ and
$T_A$ the type of $A$, supposedly matching $\AC(L)$. 
Second, the GU shows $\mcA$ and $T_A$ on its display, and
the GU operator verifies whether the aircraft $\AC(L)$ she sees on 
the parking position is indeed of airline $\mcA$ and type $T_A$. 
If yes, then she will confirm the process; otherwise she will
stop the process and raise an alarm. This can be done using the
provided input buttons on the GU TAGA controller. 
\end{measure}

\begin{measure}[`Four Eyes' Verification of AC (4EV)]
\label{m:human:four}
For increased security a member of the AC crew can accompany the GU 
operator and perform the visual verification as well.  
\end{measure}

Unintended errors of the GU operator (and AC crew member) can be kept small: 
they can be trained to keep awareness by injection of false alarms 
(similary to security screening at airports). 
Note that if $P$ is not KCI resilient then Attack~\ref{att:kci} is possible 
even when this measure is in place.



==> resil/measure-phy-cr.tex <==
\subsubsection{Physical Challenge Response}
The second measure translates the standard scheme of challenge response
authentication into the concept of \emph{physical challenge (cyber) response}:
the GU sends a challenge via the physical connection, e.g.\ encoded 
in a pattern of pulsating flow, which the AC must answer via the 
cyber channel. Thereby the physical
connection is directly bound into the KE process. 
Note that physical challenge response only counters Imp2GU attacks, 
and can be undermined by a MitM attacker. 
%In contrast to
%physical key confirmation (c.f.\ Measure~\ref{m:phyKey}) physical 
%challenge response only counters Imp2GU attacks, and can be undermined by
%a MitM attacker. The advantage is that it works directly and not
%via an alarm raised by the AC. 

\begin{figure}
\input{figures/fig-measure-phy}
\caption{\label{fig:meas:phyCR} Physical Challenge Response}
\end{figure}

\begin{measure}[Physical Challenge Response (PCR)]
\label{m:phyCR}
%Similarly to Measure~\ref{m:phyKey} 
We assume that the airpacks are 
equipped with mass airflow sensors that can detect a pattern of
airflow changes and report it to the AC controller.
Then a phase of physical challenge response can be included 
between the setup phase and the M2M phase as illustrated in 
Fig.~\ref{fig:meas:phyCR}.
$G$ generates a random number of a fixed size, say $N_G$, and encodes 
this into a pattern of pulsating airflow.
$A$ reads the physical signal by the airflow sensors and decodes it
back into a number, say $N_\nread$. $A$ then responds by sending 
$N_\nread$
back to $G$ via the cyber channel. $G$ checks whether $N_\nread = N_G$.
If this is true then $G$ concludes that it speaks to 
$\AC(L)$: only the AC that is physically connected
to the GU could have known $N_G$. If the numbers don't agree $G$ stops
and raises an alarm.
\end{measure}

The space of nonces must be sufficiently large to reduce the risk of
guessing attacks: even when the attacker cannot receive the physical
signal he can always guess the nonce $N_G$ and send it back via a cyber 
channel he has established with the GU by an impersonation attack.
This brings about a trade-off between security and efficiency. For
example:
say the physical channel allows a binary encoding of numbers in terms of
high and low airflow (e.g.\ using stuffing to synchronize). Say an  
encoded bit requires 2 seconds to be
transmitted, and a challenge shall maximally take 10 (or 20) seconds to be
transmitted. Then one can use a space of 32 (or 1024) nonces, and the
attacker has a 1/32 (or 1/1024) chance to guess correctly. 




==> resil/measure-time.tex <==
\subsubsection{Time-based Detection}
\label{s:auth:measure:time}

The third measure makes use of the awareness of the local AC that something
is wrong when it is not able to complete a started TAGA session, 
say for service $S$, within the expected amount of time. Naturally, 
this detection measure is limited to the case when the attacker is not
able to ensure that the
AC does have a successful session for $S$ (via MitM or mismatch
diversion). 
 
With respect to TAGA pairing for a fixed service $S$, 
let $t$ be the time required from 
the point after the second NFC tap at the AC up to the point when
the AC has received the Finish message. Let $t_\mmax$ be the expected maximal
value for $t$. Say the AC controller has received a TAGA request for 
service $S$, and starts a corresponding session. It makes sense that 
the AC shall abort this session if it does not receive the corresponding
Finish message within $t_\mmax$. In addition, the AC can raise an alarm 
to alert the GU operator, who in turn can abort the TAGA session at the GU. 

Say the attacker carries out an Imp2GU attack. Then the GU might start 
safety-critical processing with impact on the AC before the GU operator
had a chance to abort the TAGA session at the GU based on the alarm
mechanism. To prevent this the GU can be programmed to wait with 
safety-critical processing until it can be sure that no alarm will occur. 
With respect to our fixed service $S$, let $t'$ be 
the time required from the point after the second NFC tap at the AC
up to the point when the GU has received the final
NFC tap. Let $t'_\mmin$ be the expected minimal 
value for $t'$. Let $t^\mstop$ be the time the operator needs to carry out an
emergency stop once he has heard the alarm, and let $t^\mstop_\mmax$ be the
expected maximal value for $t^\mstop$. Then clearly we have: 
if the TAGA session of the GU has not been stopped within
$t_\mwait = t_\mmax - t'_\mmin + t^\mstop_\mmax$ time after it has received 
the final NFC tap then the local AC must have successfully established 
a session for $S$, and the GU can start with safety-critical processing.

Not that this argument relies on the fact that the AC has indeed
received a request for $S$ with the
second NFC tap. The latter is not necessarily given: e.g.\ the attacker 
might swap the request with another request as illustrated in 
Attack~\ref{att:agreem}. But we can enforce this by letting the GU operator 
carry out a `two eye' verification that the request
received by the AC coincides with a TAGA request for the service $S$ she
is pairing up (similarly to Measure~\ref{m:human:two}). 

%The GU can defer safety-critical settings until this time.
%For this to work as a measure against Imp2GU the AC needs to be aware 
%that a KE process for $S$ is underway. This can be implemented by a display.

\begin{figure}
\input{figures/fig-measure-time}
\caption{\label{fig:m:time} Time-based detection}
\end{figure}
  
\begin{measure}[Time-based Detection (TD)]
Let $t_\mmax$ and $t_\mwait$ be given as above. We assume the TAGA 
controller of the AC is equipped with a display and two input buttons: 
one to confirm, and the second to stop the process and raise an alarm. 
Then TAGA can be extended by a time-based detection process as illustrated in 
Fig.~\ref{fig:m:time}. The operator verifies with the help of the
display that the request received by the AC via the second NFC tap
coincides with a TAGA request for the service $S$ she carries out.
If this is fine  the AC starts a timer, say $T_A$. If the corresponding Finish 
message is not received before $T_A$ has reached $t_\mmax$ then
$A$ will raise an alarm. This will trigger the operator to go to
$G$ and stop $G$'s TAGA session. $G$ defers any safety-critical
processes or settings until $t_\mwait$ time has passed from the
point of the third NFC tap. If no alarm has been raised and the
operator has not stopped the TAGA session by then the GU will conclude
no attack has occurred and continue as usual. 
\end{measure}

This measure comes with a trade-off between usability and 
efficiency: if $t_\mmax$
is set too large then the process takes a lot longer than necessary; 
if $t_\mmax$ is set too small then there will be too many false 
positives and/or pressure on the operator to hurry. 
$t_\mmax^\mstop$ can be chosen to be small when the operator is 
required to stay close to the GU.


==> resil/measures.tex <==
\subsection{Local Process Measures}

Let $A$ and $G$ be a TAGA instance at a parking slot $L$, and
assume that the underlying protocol is secure and resilient.
If the attacker can only use LTKCs of domains other than that of 
$G$ and $A$, what can he still achieve with them? 
He can mount an Imp2GU attack with any compromised
AC certificate (as we have seen earlier). However, he is not able to obtain 
an Imp2AC or MitM attack since the AC can check whether the 
GU certificate is of the proper domain: of the local airport. 
Hence, the problem of obtaining domain-reliant resilient TAGA 
reduces to finding measures against `Impersonation to GU' attacks. 
We now discuss several such methods. 

\removed{
However, the challenge of impersonation can only be tackled by
additional process measures. 
We now discuss several methods of how `Impersonation to GU'
attacks (based on LTKC AC) can be detected (in combination with
KCIR/KCAR) before the GU sets
off any safety-critical services. Methods for the other direction
are analogous.}

\removed{
secure against Imp2GU.

LTKC A: Imp2GU is not avoidable by protocol improvements. (mismatch?)
now measures that together with protocol props will detec/contain risk.

safety-critical attack states.

Notation: $S:measure$ measures can be service specific.
}

%\input{auth/design-phy} move

\input{resil/measure-human}
\input{resil/measure-phy-cr}
\input{resil/measure-time}


==> resil/proofs-measure.tex <==

\begin{proof}[physical challenge response]
Someone has replied correctly via channel secured by $K$. Only $A_L$
could have known the nonce. Hence, $A$ must know $K$. 
or also attacker. must know $K$. same
same key.
\end{proof}

\begin{proof}[physical key confirmation]
G sends hash of public key and parameters. A compares alarm.
only with alarm
\end{proof}

\begin{proof}[time]

\end{proof}

\begin{proof}
Someone has confirmed $K$. This must be $A_L$ or the attacker must
know $K$.  By protocol 
the key can only be shared by someone who knows
the private key corresponding to $W_A$ used in the computation of $G$. 
We have checked that 
$W_A$ corresponds to the type of $\AC(L)$. Hence, if the attacker
knows $K$ then he must have obtained a LTKC of the domain of $A_L$.

For an Imp2GU the attacker requires a certificate/LTKCS of an AC.
could be inner domain mismatch
does not require $A$ does not know K. but requires 
can't be another A.
\end{proof}

either $A$ at $L$ or the attacker.

Kci

\begin{proof}
$G_L$: Someone has confirmed $K$ for $S$. $A_L$ has received
a request for $S$, and would have issued an alarm by now if it
didn't have key confirmation. Hence, the key $K$ $A_L$ has for
$S$, say $K'$, must match with the key confirmation it received.

Hence, either $K = K'$ and $A$ knows $K$ or the attacker knows 
both $K$ and $K'$.  However, for a Imp2AC attack the attacker
requires a certificate/LTKCS of $G$ domain.
\end{proof}


==> resil/resProt.tex <==
\subsubsection{Resilient TAGA Protocol}
Thereby motivated we define:

\begin{definition}
An AKE protocol that is secure for authenicated TAGA is also
\emph{resilient for TAGA} when it further guarantees KCI resilience, 
LTKC resilience of authentication, and LTKC resilience
against passive attackers.
\end{definition}


==> resil/resil-other.tex <==

\subsection{Other resilience}

Moreover, both designs guarantee resilience against parallel attacks
by ...:



==> resil/tab-localPKI.tex <==
\begin{enumerate}
\item It is the responsibility of the airport to ensure that
   each GU in their domain only presents a valid/safe certificate           
   to the AC during a TAGA process rather than the AC's responsibility
   to check whether the GU's certificate has been revoked. And similarly
   for the other direction.

\item Every airport is responsible to provide their root certificate
  to any airline that participates in TAGA (with some public or
gonvernmental record thereof). 
But it is the airline's responsibility to install the
  thus provided valid root certificates in it's AC's endpoints.
\item It is the responsibility of the domain to put measures in place
 so that their key management is provably secure against LTKCs of
 their domain or comes close and/LTKCs of their domain are 
  detected quickly. 
\item If an incidence happens at a location $L$ then it can be traced
 whether this is due to a LTKC, in which case it can also be 
  traced to the responsible domain. 
\end{enumerate}



==> setup-2/attack-states.tex <==

%\parbox{\columnwidth}{
Let $G$ be a GU to carry out service $S$ at $L$. 
Assume $G$ believes it shares a secure channel with $\AC(L)$
for M2M communication on $S$. We say $G$ is in attack state  

\begin{enumerate}
\item \emph{full attacker control} 
  ($\att$) if indeed $G$ shares the channel with the attacker;

\item \emph{location mismatch} ($\mmLoc$) if indeed $G$ shares the channel with an AC 
    at parking position $L' \not = L$, who agrees the channel is for
    service $S$;

\item \emph{service mismatch} ($\mmSer$) if indeed $G$ shares the channel with $\AC(L)$ but $\AC(L)$
      believes the channel is for service $S' \not = S$.

\item \emph{location \& service mismatch} ($\mmLocSer$)
       if indeed $G$ shares the channel with an AC at parking
      position $L' \not = L$, who believes the channel is for 
      service $S' \not = S$.
\end{enumerate}

%In (2)-(4) we assume the channel is secure from the attacker.
Let $A$ be an AC to be serviced at $L$. Assume $A$ believes
it shares a secure channel with some GU at $L$ %$\GU(L, S)$ for 
for M2M communication on $S$. We say $A$ is wrt $S$ in attack state

\begin{enumerate}
\item \emph{full attacker control} ($\att$) if indeed
      $A$ shares the channel with the attacker;

\item \emph{location mismatch} ($\mmLoc$): if indeed $A$ shares the 
     channel with a GU at 
     parking position $L' \not = L$, who agrees the channel is for
     service $S$; 

\item \emph{service mismatch} ($\mmSer$): if indeed $A$ shares the 
      channel with some GU $G$ at $L$ but
      $G$ believes the channel is for service $S' \not = S$.

\item \emph{location \& service mismtach} ($\mmLocSer$): if
      indeed $A$ shares the channel with a GU at parking
      position $L' \not = L$, who believes the channel is for 
      service $S' \not = S$.
\end{enumerate}
We denote the set of such attack states of an AC or GU by $\statesA$.

Let $S$ be a service involving two GUs. The \emph{attack state of channels
on $S$ with impact on $L$} is specified as a pair $(\cs_G, \cs_A) 
\subseteq \{\undef, \none\} \cup \statesG \times \{\none\} \cup \statesA$ 
such that
\begin{enumerate}
\item if $\AC(L)$ has established a channel for $S$ then
      $\cs_A$ is the attack state of this channel, and otherwise
      $\cs_A = \none$;
\item if $\AC(L)$ is physically connected to some GU for $S$, say $G_S$,
      \begin{itemize} 
      \item then 
       if $G_S$ has established a channel for $S$ then $\cs_G$ is
      the attack state of this channel, and otherwise $\cs_G = \none$;
     \item otherwise $\cs_G = \undef$.
    \end{itemize}
\end{enumerate}



==> setup-2/safety-long.tex <==
\subsection{Potential M2M Attack States and Safety Impact}

\label{s:goals:safety}

\begin{table}
\input{goals/attack-states}
\caption{\label{tab:attackStates} Potential M2M Attack States}
\end{table}

Let $L$ be a parking position, and $S$ a ground service being or to be 
carried out at $L$. Assume an attacker intends to cause harm at $L$ by 
undermining the M2M communication on $S$. I.e., the goal of the attacker 
is to compromise communication channels that impact on $S$ in some way, 
and to thereby reach an attack state from which he can directly 
or indirectly induce the AC or GU control of $S$ to actuate some 
unsafe physical effect 
at $L$.  We have identified the set of \emph{potential} attack states
such an attacker could try to reach: the definition is provided
in Table~\ref{tab:attackStates} for services with one GU, and 
the generalization to services with $n$ GUs can be found in 
App.~\ref{app:safety}.
Our definition underlies the following assumption, which 
is motivated by the fact that usually 
the physical control of the GU is only activated as the last step 
of the physical setup (c.f.\ Section~\ref{s:taga:services}). 

\begin{assumption}
As long as the GU has not completed the physical setup process for
the service it provides its own physical control cannot be the 
cause of any safety
impact (even if the GU has a compromised communication channel). 
\end{assumption}

Then to capture the potential attack states we need 
to take into account 
all channels that $A$ believes it has for $S$, and
the channel that any GU that
is physically connected to $A$ believes it has for $S$, as well as the absence 
of such channels. Note that a channel can
be under the entire control of the attacker (e.g.\ when the
sesssion key has been compromised) or undermined in a more subtle way:
e.g.\ when the AC is connected to a GU at a different location or to 
a GU of a different service.

We now discuss the most relevant attack states and the safety 
impact for air conditioning and fuelling. This is in preparation
for our resilience analysis, which will uncover how the relevant
attack states are reached when certain security incidences
have taken place. Moreover, the examples illustrate that the
security properties are not only sufficient for secure setup
but also necessary. (The special case of identity mismatch attacks
will be discussed below.)
%has no safety impact, but discussed below.
%
In the following, let $L$ be a parking position, $A$ be the AC at
$L$, and $G_S$ a GU for service $S$ at $L$. C.f.\ Fig.~\ref{fig:astates} 
for illustration.

\begin{figure*}
\begin{tabular}{ccc}
\subfloat[MitM]{
\input{figures/att-mitm}}
&
\subfloat[Imp2GU]{
\input{figures/att-imp2gu}}
&
\subfloat[Imp2AC]{
\input{figures/att-imp2ac}}
\\
\subfloat[Imp2GU with location mismatch of AC]{
\input{figures/att-imp2gu-div}}
&
\subfloat[Location mismatch of GU]{
\input{figures/att-mism-gu}}
& 
\begin{tabular}[b]{c}
\subfloat[Service mismach of GU]{
\input{figures/att-mism-ser-gu}}
\\
\subfloat[Service mismatch of AC]{
\input{figures/att-mism-ser-ac}}
\end{tabular}
\end{tabular}

\caption{\label{fig:astates} M2M attack states }
\end{figure*} 



\subsubsection{Man-in-the-Middle (MitM)} The most serious attack state
is $(\att, \att)$: it means the attacker has established himself as 
the man-in-the-middle between $A$ and $G_S$; he can insert, delete 
or modify any messages as he pleases. 
%Typically the attacker will realize this
%by setting up two connections, one with $A$ and one with $G_S$.
As our examples show the safety impact is high for air conditioning 
but not so for fuelling due to inbuilt safety measures.
% governed by the
%physical process is protected by measures of the AC.

\begin{example}[Air Conditioning]
\label{ex:MitM:aircond}
The attacker can forge airflow parameters and sensor values
that will induce $G_S$ to apply air pressure and temperature
unsuitable to $A$. This can be highly damaging: if the cooling process 
is too fast, water in the pipes can quickly become frozen and 
clog up the pipes. This can happen very quickly: e.g. with the lowest 
inlet temperature within 30 seconds, with safety considerations 
still within 100 seconds. The resulting backflow will be detected by the GU.
However, in the worst case pipes might already have burst. In any case 
the pipes have to be checked for damage afterwards, which is a costly procedure.
In the worst case, the attacker could try to optimize the attack based
on the sensor values sent by $A$: he could try to control the airflow in
a way that maximizes the strain on the pipes without this being
detected during service time but with a high risk that pipes burst during 
flight.
\end{example}

\begin{example}[Fuelling]
\label{ex:MitM:fuelling}
The attacker can forge fuel orders, and induce the fuel truck to
load an insufficient or surplus amount of fuel. While this can be highly 
disruptive there is no safety impact. Since the AC measures the fuel 
itself $A$ will notice if the loaded fuel is not sufficient. Moreover, 
if the attacker tries to cause spillage (and hence a fire
hazard) by too large a fuel order this will not succeed either since
backflow will stop the pump of the fuel truck. 
\end{example}

\subsubsection{Impersonation to GU (Imp2GU)} 
Another serious attack state is $(\att, \neg \att)$. 
This allows the attacker to impersonate $A$ to $G_S$ (but not
vice versa): he can feed any information he likes to $G_S$ while 
$G_S$ thinks this information stems from $A$ and adjusts the 
service correspondingly. The safety impact is potentially high.

\begin{example}[Air Conditioning]
The attacker feeds in airflow parameters and sensor values,
and $G_S$ will control the airflow based on this information.
Since the air supply leads directly into the mixer unit of the plane 
this will take immediate effect without $A$ itself having to open a valve or
the like first. Crew or ground stuff might notice that something is
wrong and switch off the air supply manually. However, as discussed in
Example~\ref{ex:MitM:aircond} damage 
can occur quickly and this might be too late. In contrast to the MitM 
attack the attacker is not able to optimize the attack based on 
sensor values from $A$.
\end{example}

\subsubsection{Imp2GU with Mismatch Diversion}
In some situations it might be beneficial for the attacker to divert 
the AC by matching it up with another GU: to reach 
attack state $(\att, \mmX)$ rather than $(\att, \none)$.
One reason is to thereby ensure that the impersonation attack 
remains undetected for longer; 
another reason is that without a successful session the 
AC might not be affected at all, perhaps because it controls a valve 
that it will not open otherwise.
 
\begin{example}[Fuelling]
When fuelling the pilot has to open the valves of the tanks before 
the fuel flow can start. Hence, as long as $A$ does not have a 
successful session for fuelling the Imp2GU attack will be detected 
early on: the fuel pump of $G_S$ will stop almost immediately due to backflow. 
However, if the attacker reaches the attack state
$(\att, \mmX)$ then $A$  will open the fuel valves, and the attacker can
make $G_S$ load fuel based on a forged order. Fortunately, in this
case there is no safety impact as explained in Example~\ref{ex:MitM:fuelling}.
\end{example}

\subsubsection{Impersonation to AC (Imp2AC)} 
When the physical control of the service lies entirely with the GU
(as with air conditioning) then the attack states $(\none, \att)$
and $(\undef, \att)$ are harmless. 
Although the attacker can feed any information he likes to
$A$ nothing will happen until a GU engages into the service. And
any GU will only do so after it has completed the physical setup 
and established a channel for the service itself. 
%Finally, crew or ground stuff will notice that something is 
%wrong. 
When the physical control lies at least partly with
the AC then this attack state can have safety impact or not, e.g.\ depending 
on whether there are inbuilt safety measures.

\begin{example}[Fuelling]
The attacker can impersonate the fuel truck and in its name report to 
$A$ that a problem has occurred. This could induce $A$ to close the
valves of the tank while in reality nothing is wrong with the
fuel truck and it keeps pumping fuel. However, this will not result 
in any safety issue since the truck will simply stop pumping due to back flow.
\end{example}

Analogously to Imp2GU, the attacker could try to reach the attack
state $(\mmX, \att)$ to combine  Imp2AC with a mismatch 
diversion of the GU. Alternatively, in this state the Imp2AC attack
could itself be the diversion to a safety-critical location mismatch attack 
as we will see next.

\subsubsection{Location Mismatch of GU}
We have already seen that mismatch attacks can be used as a diversion.
The following example of a $(\mmLoc, \ast)$ attack
illustrates that they can be safety-critical in their own right. 

\begin{example}[Air Conditioning]
Let $A'$ be an AC at another parking position $L'$ with ongoing
air conditioning service. 
Assume $A'$ is a large plane (e.g.\ an A380), and $A$ is a smaller plane
(e.g.\ an A319). Moreover, assume the attacker has obtained a
mismatch state $(\mmLoc, \ast)$ where $G_S$ is speaking to $A'$.
Hence, $A'$ will communicate its parameters for airflow to $G_S$ while
$G_S$'s air supply hose is connected to the smaller $A$. 
Since the airpacks of $A$ are smaller than those of $A'$ 
airflow parameters suitable for $A'$ can be damaging for $A$: 
the air pressure is likely to be too high and the cooling process too 
fast. As a consequence pipes of $A$ can be damaged as explained
in Example~\ref{ex:MitM:aircond}.
\end{example}

%GU mismatch same 
%Mismatch with Impersonation to AC (Imp2AC)

\subsubsection{Service Mismatch}
A service mismatch $(\mmSer, \ast)$ or $(\ast, \mmSer)$ will likely 
be noticed as soon as M2M communication starts. 
The messages will not follow the protocol the AC, and respectively 
GU expects, and hence errors will be raised: e.g.\ the AC 
provides temperature readings while the GU expects a fuel order. 
However, a service mismatch could still be employed as a diversion
to support another attack: when the only goal is that the party to divert
has established a channel for the service (because only then it will
open a valve), or when the service is such that there usually is
a delay between the point when the channel is established and the start
of the M2M communication. 

\subsubsection{Identity Mismatch}
TODO to synchronize with something in TAGA auth.

billing, (fuel) unknown-key share for location-mismatch,
talk with the one for L and S, have certificate for low S'/A 


